Counting Distinct Elements Under Person-Level Differential Privacy

We study the problem of counting the number of distinct elements in a dataset subject to the constraint of differential privacy. We consider the challenging setting of person-level DP (a.k.a. user-level DP) where each person may contribute an unbounded number of items and hence the sensitivity is unbounded. Our approach is to compute a bounded-sensitivity version of this query, which reduces to solving a max-flow problem. The sensitivity bound is optimized to balance the noise we must add to privatize the answer against the error of the approximation of the bounded-sensitivity query to the true number of unique elements.

==> figures/bounds/amazon_fashion.tex <==
\nextgroupplot [
    title=Amazon Fashion,
    xmin=-3.9, xmax=103.9,
    ymin=120.49, ymax=1513.31,
    ylabel={Distinct Count},
    legend style = {
        column sep = 10pt,
        legend columns = 2, 
        legend to name = grouplegend,
        draw=none
    }
]


\addplot [dashed, steelblue31119180]
table {%
1 1450
2 1450
3 1450
4 1450
5 1450
6 1450
7 1450
8 1450
9 1450
10 1450
11 1450
12 1450
13 1450
14 1450
15 1450
16 1450
17 1450
18 1450
19 1450
20 1450
21 1450
22 1450
23 1450
24 1450
25 1450
26 1450
27 1450
28 1450
29 1450
30 1450
31 1450
32 1450
33 1450
34 1450
35 1450
36 1450
37 1450
38 1450
39 1450
40 1450
41 1450
42 1450
43 1450
44 1450
45 1450
46 1450
47 1450
48 1450
49 1450
50 1450
51 1450
52 1450
53 1450
54 1450
55 1450
56 1450
57 1450
58 1450
59 1450
60 1450
61 1450
62 1450
63 1450
64 1450
65 1450
66 1450
67 1450
68 1450
69 1450
70 1450
71 1450
72 1450
73 1450
74 1450
75 1450
76 1450
77 1450
78 1450
79 1450
80 1450
81 1450
82 1450
83 1450
84 1450
85 1450
86 1450
87 1450
88 1450
89 1450
90 1450
91 1450
92 1450
93 1450
94 1450
95 1450
96 1450
97 1450
98 1450
99 1450
};
\addplot [densely dotted, thick, forestgreen4416044]
table {%
1 368.0
2 643.0
3 855.0
4 1014.0
5 1117.0
6 1195.0
7 1252.0
8 1290.0
9 1317.0
10 1340.0
11 1357.0
12 1373.0
13 1387.0
14 1400.0
15 1412.0
16 1420.0
17 1428.0
18 1432.0
19 1435.0
20 1438.0
21 1441.0
22 1442.0
23 1443.0
24 1444.0
25 1445.0
26 1446.0
27 1447.0
28 1448.0
29 1449.0
30 1450.0
31 1450.0
32 1450.0
33 1450.0
34 1450.0
35 1450.0
36 1450.0
37 1450.0
38 1450.0
39 1450.0
40 1450.0
41 1450.0
42 1450.0
43 1450.0
44 1450.0
45 1450.0
46 1450.0
47 1450.0
48 1450.0
49 1450.0
50 1450.0
51 1450.0
52 1450.0
53 1450.0
54 1450.0
55 1450.0
56 1450.0
57 1450.0
58 1450.0
59 1450.0
60 1450.0
61 1450.0
62 1450.0
63 1450.0
64 1450.0
65 1450.0
66 1450.0
67 1450.0
68 1450.0
69 1450.0
70 1450.0
71 1450.0
72 1450.0
73 1450.0
74 1450.0
75 1450.0
76 1450.0
77 1450.0
78 1450.0
79 1450.0
80 1450.0
81 1450.0
82 1450.0
83 1450.0
84 1450.0
85 1450.0
86 1450.0
87 1450.0
88 1450.0
89 1450.0
90 1450.0
91 1450.0
92 1450.0
93 1450.0
94 1450.0
95 1450.0
96 1450.0
97 1450.0
98 1450.0
99 1450.0
};
\addplot [densely dotted, thick, darkorange25512714]
table {%
1 333.0
2 572.0
3 763.0
4 903.0
5 1012.0
6 1097.0
7 1161.0
8 1209.0
9 1247.0
10 1275.0
11 1298.0
12 1317.0
13 1335.0
14 1351.0
15 1366.0
16 1380.0
17 1392.0
18 1401.0
19 1408.0
20 1415.0
21 1422.0
22 1428.0
23 1433.0
24 1436.0
25 1438.0
26 1440.0
27 1442.0
28 1444.0
29 1446.0
30 1447.0
31 1448.0
32 1449.0
33 1450.0
34 1450.0
35 1450.0
36 1450.0
37 1450.0
38 1450.0
39 1450.0
40 1450.0
41 1450.0
42 1450.0
43 1450.0
44 1450.0
45 1450.0
46 1450.0
47 1450.0
48 1450.0
49 1450.0
50 1450.0
51 1450.0
52 1450.0
53 1450.0
54 1450.0
55 1450.0
56 1450.0
57 1450.0
58 1450.0
59 1450.0
60 1450.0
61 1450.0
62 1450.0
63 1450.0
64 1450.0
65 1450.0
66 1450.0
67 1450.0
68 1450.0
69 1450.0
70 1450.0
71 1450.0
72 1450.0
73 1450.0
74 1450.0
75 1450.0
76 1450.0
77 1450.0
78 1450.0
79 1450.0
80 1450.0
81 1450.0
82 1450.0
83 1450.0
84 1450.0
85 1450.0
86 1450.0
87 1450.0
88 1450.0
89 1450.0
90 1450.0
91 1450.0
92 1450.0
93 1450.0
94 1450.0
95 1450.0
96 1450.0
97 1450.0
98 1450.0
99 1450.0
};
\path [fill=crimson2143940, fill opacity=0.2]
(axis cs:1,179.9)--
(axis cs:1,198.0)--
(axis cs:2,305.1)--
(axis cs:3,388.1)--
(axis cs:4,460.0)--
(axis cs:5,515.0)--
(axis cs:6,566.1)--
(axis cs:7,614.0)--
(axis cs:8,658.0)--
(axis cs:9,698.0)--
(axis cs:10,738.1)--
(axis cs:11,770.1)--
(axis cs:12,801.0)--
(axis cs:13,830.0)--
(axis cs:14,864.0)--
(axis cs:15,887.0)--
(axis cs:16,918.1)--
(axis cs:17,938.1)--
(axis cs:18,961.1)--
(axis cs:19,977.1)--
(axis cs:20,1001.1)--
(axis cs:21,1028.0)--
(axis cs:22,1043.0)--
(axis cs:23,1063.0)--
(axis cs:24,1078.2)--
(axis cs:25,1096.0)--
(axis cs:26,1111.1)--
(axis cs:27,1131.0)--
(axis cs:28,1142.0)--
(axis cs:29,1158.0)--
(axis cs:30,1171.0)--
(axis cs:31,1181.1)--
(axis cs:32,1191.0)--
(axis cs:33,1203.0)--
(axis cs:34,1212.1)--
(axis cs:35,1222.1)--
(axis cs:36,1227.2)--
(axis cs:37,1240.1)--
(axis cs:38,1247.0)--
(axis cs:39,1258.0)--
(axis cs:40,1263.1)--
(axis cs:41,1273.1)--
(axis cs:42,1276.1)--
(axis cs:43,1287.0)--
(axis cs:44,1291.1)--
(axis cs:45,1298.0)--
(axis cs:46,1300.0)--
(axis cs:47,1309.0)--
(axis cs:48,1311.2)--
(axis cs:49,1317.0)--
(axis cs:50,1320.0)--
(axis cs:51,1325.0)--
(axis cs:52,1332.0)--
(axis cs:53,1334.0)--
(axis cs:54,1339.1)--
(axis cs:55,1342.0)--
(axis cs:56,1344.0)--
(axis cs:57,1345.1)--
(axis cs:58,1351.1)--
(axis cs:59,1353.0)--
(axis cs:60,1357.0)--
(axis cs:61,1360.1)--
(axis cs:62,1364.0)--
(axis cs:63,1365.1)--
(axis cs:64,1368.1)--
(axis cs:65,1372.0)--
(axis cs:66,1373.0)--
(axis cs:67,1378.1)--
(axis cs:68,1377.1)--
(axis cs:69,1381.0)--
(axis cs:70,1384.0)--
(axis cs:71,1385.2)--
(axis cs:72,1387.0)--
(axis cs:73,1393.0)--
(axis cs:74,1396.0)--
(axis cs:75,1397.0)--
(axis cs:76,1397.1)--
(axis cs:77,1401.0)--
(axis cs:78,1403.0)--
(axis cs:79,1404.0)--
(axis cs:80,1407.1)--
(axis cs:81,1410.0)--
(axis cs:82,1412.0)--
(axis cs:83,1413.0)--
(axis cs:84,1415.0)--
(axis cs:85,1416.0)--
(axis cs:86,1419.0)--
(axis cs:87,1421.1)--
(axis cs:88,1423.0)--
(axis cs:89,1423.0)--
(axis cs:90,1424.0)--
(axis cs:91,1427.0)--
(axis cs:92,1428.0)--
(axis cs:93,1427.0)--
(axis cs:94,1431.0)--
(axis cs:95,1430.0)--
(axis cs:96,1431.0)--
(axis cs:97,1432.0)--
(axis cs:98,1432.0)--
(axis cs:99,1434.1)--
(axis cs:99,1424.9)--
(axis cs:98,1423.0)--
(axis cs:97,1422.0)--
(axis cs:96,1421.0)--
(axis cs:95,1421.0)--
(axis cs:94,1420.0)--
(axis cs:93,1418.9)--
(axis cs:92,1416.9)--
(axis cs:91,1415.0)--
(axis cs:90,1413.0)--
(axis cs:89,1412.0)--
(axis cs:88,1410.0)--
(axis cs:87,1409.0)--
(axis cs:86,1406.0)--
(axis cs:85,1405.0)--
(axis cs:84,1402.9)--
(axis cs:83,1401.9)--
(axis cs:82,1398.0)--
(axis cs:81,1396.0)--
(axis cs:80,1394.0)--
(axis cs:79,1390.0)--
(axis cs:78,1387.9)--
(axis cs:77,1386.0)--
(axis cs:76,1385.0)--
(axis cs:75,1379.9)--
(axis cs:74,1377.0)--
(axis cs:73,1377.0)--
(axis cs:72,1373.0)--
(axis cs:71,1370.0)--
(axis cs:70,1367.0)--
(axis cs:69,1366.0)--
(axis cs:68,1363.0)--
(axis cs:67,1361.0)--
(axis cs:66,1358.0)--
(axis cs:65,1354.9)--
(axis cs:64,1350.0)--
(axis cs:63,1348.0)--
(axis cs:62,1345.9)--
(axis cs:61,1342.0)--
(axis cs:60,1339.9)--
(axis cs:59,1335.9)--
(axis cs:58,1333.0)--
(axis cs:57,1331.0)--
(axis cs:56,1325.0)--
(axis cs:55,1321.0)--
(axis cs:54,1320.8)--
(axis cs:53,1315.0)--
(axis cs:52,1310.9)--
(axis cs:51,1305.9)--
(axis cs:50,1300.0)--
(axis cs:49,1294.8)--
(axis cs:48,1290.9)--
(axis cs:47,1286.9)--
(axis cs:46,1281.8)--
(axis cs:45,1275.0)--
(axis cs:44,1268.0)--
(axis cs:43,1265.0)--
(axis cs:42,1252.0)--
(axis cs:41,1247.9)--
(axis cs:40,1240.0)--
(axis cs:39,1236.0)--
(axis cs:38,1224.0)--
(axis cs:37,1218.0)--
(axis cs:36,1205.0)--
(axis cs:35,1201.0)--
(axis cs:34,1188.9)--
(axis cs:33,1178.0)--
(axis cs:32,1165.9)--
(axis cs:31,1152.9)--
(axis cs:30,1145.9)--
(axis cs:29,1128.9)--
(axis cs:28,1119.9)--
(axis cs:27,1099.9)--
(axis cs:26,1088.0)--
(axis cs:25,1065.0)--
(axis cs:24,1052.9)--
(axis cs:23,1038.0)--
(axis cs:22,1018.9)--
(axis cs:21,1000.0)--
(axis cs:20,979.0)--
(axis cs:19,949.9)--
(axis cs:18,935.0)--
(axis cs:17,910.0)--
(axis cs:16,882.0)--
(axis cs:15,855.9)--
(axis cs:14,830.8)--
(axis cs:13,801.0)--
(axis cs:12,771.0)--
(axis cs:11,734.9)--
(axis cs:10,701.8)--
(axis cs:9,664.0)--
(axis cs:8,627.0)--
(axis cs:7,583.0)--
(axis cs:6,534.9)--
(axis cs:5,490.0)--
(axis cs:4,432.0)--
(axis cs:3,367.0)--
(axis cs:2,283.0)--
(axis cs:1,179.9)--
cycle;
\addplot [dashdotted, thick, crimson2143940]
table {%
1 188.5
2 295.0
3 376.5
4 445.0
5 501.0
6 551.5
7 599.5
8 642.5
9 681.0
10 719.0
11 752.0
12 784.0
13 817.0
14 846.0
15 872.0
16 899.0
17 922.0
18 949.0
19 964.5
20 990.0
21 1011.5
22 1032.0
23 1049.5
24 1067.0
25 1082.0
26 1100.0
27 1114.0
28 1129.0
29 1143.5
30 1157.0
31 1169.0
32 1177.0
33 1190.0
34 1200.5
35 1211.0
36 1219.0
37 1228.0
38 1237.0
39 1246.0
40 1251.0
41 1258.0
42 1265.0
43 1274.0
44 1281.0
45 1284.0
46 1290.0
47 1297.0
48 1302.0
49 1306.0
50 1310.5
51 1316.0
52 1322.5
53 1324.5
54 1329.0
55 1331.0
56 1334.0
57 1338.0
58 1342.0
59 1346.0
60 1348.0
61 1352.0
62 1354.5
63 1357.0
64 1359.0
65 1363.0
66 1365.0
67 1369.0
68 1370.0
69 1374.0
70 1374.5
71 1379.0
72 1381.0
73 1384.0
74 1385.0
75 1388.0
76 1391.0
77 1393.0
78 1396.0
79 1397.0
80 1401.0
81 1403.0
82 1405.0
83 1407.5
84 1409.0
85 1411.0
86 1413.0
87 1415.0
88 1417.0
89 1418.5
90 1419.0
91 1421.0
92 1422.5
93 1423.0
94 1425.0
95 1425.0
96 1426.0
97 1427.0
98 1428.0
99 1429.0
};
\path [fill=darkgray176, fill opacity=0.2]
(axis cs:1,180.9)--
(axis cs:1,201.0)--
(axis cs:2,421.1)--
(axis cs:3,619.1)--
(axis cs:4,784.0)--
(axis cs:5,917.2)--
(axis cs:6,1023.1)--
(axis cs:7,1108.1)--
(axis cs:8,1175.2)--
(axis cs:9,1227.1)--
(axis cs:10,1267.0)--
(axis cs:11,1295.1)--
(axis cs:12,1321.0)--
(axis cs:13,1339.1)--
(axis cs:14,1357.1)--
(axis cs:15,1373.0)--
(axis cs:16,1388.0)--
(axis cs:17,1397.0)--
(axis cs:18,1408.0)--
(axis cs:19,1416.1)--
(axis cs:20,1424.0)--
(axis cs:21,1429.0)--
(axis cs:22,1434.0)--
(axis cs:23,1438.0)--
(axis cs:24,1441.0)--
(axis cs:25,1443.0)--
(axis cs:26,1445.0)--
(axis cs:27,1445.0)--
(axis cs:28,1446.1)--
(axis cs:29,1447.1)--
(axis cs:30,1448.1)--
(axis cs:31,1450.0)--
(axis cs:32,1450.0)--
(axis cs:33,1450.0)--
(axis cs:34,1450.0)--
(axis cs:35,1450.0)--
(axis cs:36,1450.0)--
(axis cs:37,1450.0)--
(axis cs:38,1450.0)--
(axis cs:39,1450.0)--
(axis cs:40,1450.0)--
(axis cs:41,1450.0)--
(axis cs:42,1450.0)--
(axis cs:43,1450.0)--
(axis cs:44,1450.0)--
(axis cs:45,1450.0)--
(axis cs:46,1450.0)--
(axis cs:47,1450.0)--
(axis cs:48,1450.0)--
(axis cs:49,1450.0)--
(axis cs:50,1450.0)--
(axis cs:51,1450.0)--
(axis cs:52,1450.0)--
(axis cs:53,1450.0)--
(axis cs:54,1450.0)--
(axis cs:55,1450.0)--
(axis cs:56,1450.0)--
(axis cs:57,1450.0)--
(axis cs:58,1450.0)--
(axis cs:59,1450.0)--
(axis cs:60,1450.0)--
(axis cs:61,1450.0)--
(axis cs:62,1450.0)--
(axis cs:63,1450.0)--
(axis cs:64,1450.0)--
(axis cs:65,1450.0)--
(axis cs:66,1450.0)--
(axis cs:67,1450.0)--
(axis cs:68,1450.0)--
(axis cs:69,1450.0)--
(axis cs:70,1450.0)--
(axis cs:71,1450.0)--
(axis cs:72,1450.0)--
(axis cs:73,1450.0)--
(axis cs:74,1450.0)--
(axis cs:75,1450.0)--
(axis cs:76,1450.0)--
(axis cs:77,1450.0)--
(axis cs:78,1450.0)--
(axis cs:79,1450.0)--
(axis cs:80,1450.0)--
(axis cs:81,1450.0)--
(axis cs:82,1450.0)--
(axis cs:83,1450.0)--
(axis cs:84,1450.0)--
(axis cs:85,1450.0)--
(axis cs:86,1450.0)--
(axis cs:87,1450.0)--
(axis cs:88,1450.0)--
(axis cs:89,1450.0)--
(axis cs:90,1450.0)--
(axis cs:91,1450.0)--
(axis cs:92,1450.0)--
(axis cs:93,1450.0)--
(axis cs:94,1450.0)--
(axis cs:95,1450.0)--
(axis cs:96,1450.0)--
(axis cs:97,1450.0)--
(axis cs:98,1450.0)--
(axis cs:99,1450.0)--
(axis cs:99,1450.0)--
(axis cs:98,1450.0)--
(axis cs:97,1450.0)--
(axis cs:96,1450.0)--
(axis cs:95,1450.0)--
(axis cs:94,1450.0)--
(axis cs:93,1450.0)--
(axis cs:92,1450.0)--
(axis cs:91,1450.0)--
(axis cs:90,1450.0)--
(axis cs:89,1450.0)--
(axis cs:88,1450.0)--
(axis cs:87,1450.0)--
(axis cs:86,1450.0)--
(axis cs:85,1450.0)--
(axis cs:84,1450.0)--
(axis cs:83,1450.0)--
(axis cs:82,1450.0)--
(axis cs:81,1450.0)--
(axis cs:80,1450.0)--
(axis cs:79,1450.0)--
(axis cs:78,1450.0)--
(axis cs:77,1450.0)--
(axis cs:76,1450.0)--
(axis cs:75,1450.0)--
(axis cs:74,1450.0)--
(axis cs:73,1450.0)--
(axis cs:72,1450.0)--
(axis cs:71,1450.0)--
(axis cs:70,1450.0)--
(axis cs:69,1450.0)--
(axis cs:68,1450.0)--
(axis cs:67,1450.0)--
(axis cs:66,1450.0)--
(axis cs:65,1450.0)--
(axis cs:64,1450.0)--
(axis cs:63,1450.0)--
(axis cs:62,1450.0)--
(axis cs:61,1450.0)--
(axis cs:60,1450.0)--
(axis cs:59,1450.0)--
(axis cs:58,1450.0)--
(axis cs:57,1450.0)--
(axis cs:56,1450.0)--
(axis cs:55,1450.0)--
(axis cs:54,1450.0)--
(axis cs:53,1450.0)--
(axis cs:52,1450.0)--
(axis cs:51,1450.0)--
(axis cs:50,1450.0)--
(axis cs:49,1450.0)--
(axis cs:48,1450.0)--
(axis cs:47,1450.0)--
(axis cs:46,1450.0)--
(axis cs:45,1450.0)--
(axis cs:44,1450.0)--
(axis cs:43,1450.0)--
(axis cs:42,1450.0)--
(axis cs:41,1450.0)--
(axis cs:40,1450.0)--
(axis cs:39,1450.0)--
(axis cs:38,1450.0)--
(axis cs:37,1450.0)--
(axis cs:36,1450.0)--
(axis cs:35,1450.0)--
(axis cs:34,1450.0)--
(axis cs:33,1449.0)--
(axis cs:32,1447.0)--
(axis cs:31,1447.0)--
(axis cs:30,1446.0)--
(axis cs:29,1444.9)--
(axis cs:28,1444.0)--
(axis cs:27,1442.0)--
(axis cs:26,1441.0)--
(axis cs:25,1438.0)--
(axis cs:24,1436.0)--
(axis cs:23,1433.0)--
(axis cs:22,1428.0)--
(axis cs:21,1422.0)--
(axis cs:20,1415.0)--
(axis cs:19,1409.0)--
(axis cs:18,1399.9)--
(axis cs:17,1389.0)--
(axis cs:16,1378.0)--
(axis cs:15,1362.0)--
(axis cs:14,1345.9)--
(axis cs:13,1328.9)--
(axis cs:12,1307.0)--
(axis cs:11,1283.9)--
(axis cs:10,1250.0)--
(axis cs:9,1207.9)--
(axis cs:8,1157.9)--
(axis cs:7,1090.0)--
(axis cs:6,1003.0)--
(axis cs:5,894.0)--
(axis cs:4,761.0)--
(axis cs:3,592.0)--
(axis cs:2,397.0)--
(axis cs:1,180.9)--
cycle;
% \addplot [thick, darkgray176]
% table {%
% 1 190.5
% 2 410.5
% 3 606.0
% 4 772.0
% 5 905.0
% 6 1013.0
% 7 1099.5
% 8 1167.0
% 9 1218.0
% 10 1258.0
% 11 1290.0
% 12 1313.0
% 13 1334.0
% 14 1351.5
% 15 1367.0
% 16 1382.0
% 17 1393.0
% 18 1404.0
% 19 1413.0
% 20 1419.0
% 21 1426.0
% 22 1431.0
% 23 1435.5
% 24 1439.0
% 25 1440.0
% 26 1443.0
% 27 1444.0
% 28 1445.0
% 29 1446.0
% 30 1447.0
% 31 1448.0
% 32 1449.0
% 33 1450.0
% 34 1450.0
% 35 1450.0
% 36 1450.0
% 37 1450.0
% 38 1450.0
% 39 1450.0
% 40 1450.0
% 41 1450.0
% 42 1450.0
% 43 1450.0
% 44 1450.0
% 45 1450.0
% 46 1450.0
% 47 1450.0
% 48 1450.0
% 49 1450.0
% 50 1450.0
% 51 1450.0
% 52 1450.0
% 53 1450.0
% 54 1450.0
% 55 1450.0
% 56 1450.0
% 57 1450.0
% 58 1450.0
% 59 1450.0
% 60 1450.0
% 61 1450.0
% 62 1450.0
% 63 1450.0
% 64 1450.0
% 65 1450.0
% 66 1450.0
% 67 1450.0
% 68 1450.0
% 69 1450.0
% 70 1450.0
% 71 1450.0
% 72 1450.0
% 73 1450.0
% 74 1450.0
% 75 1450.0
% 76 1450.0
% 77 1450.0
% 78 1450.0
% 79 1450.0
% 80 1450.0
% 81 1450.0
% 82 1450.0
% 83 1450.0
% 84 1450.0
% 85 1450.0
% 86 1450.0
% 87 1450.0
% 88 1450.0
% 89 1450.0
% 90 1450.0
% 91 1450.0
% 92 1450.0
% 93 1450.0
% 94 1450.0
% 95 1450.0
% 96 1450.0
% 97 1450.0
% 98 1450.0
% 99 1450.0
% };





\addlegendentry{true value}
\addlegendentry{matching algorithm}
\addlegendentry{greedy algorithm}
\addlegendentry{sampling algorithm}
% \addlegendentry{iterative algorithm}

==> figures/bounds/amazon_industrial.tex <==
\nextgroupplot [
    title=Amazon Industrial,
    xmin=-3.9, xmax=103.9,
    ymin=1077.98, ymax=38359.62,
]
\addplot [dashed, steelblue31119180]
table {%
1 36665
2 36665
3 36665
4 36665
5 36665
6 36665
7 36665
8 36665
9 36665
10 36665
11 36665
12 36665
13 36665
14 36665
15 36665
16 36665
17 36665
18 36665
19 36665
20 36665
21 36665
22 36665
23 36665
24 36665
25 36665
26 36665
27 36665
28 36665
29 36665
30 36665
31 36665
32 36665
33 36665
34 36665
35 36665
36 36665
37 36665
38 36665
39 36665
40 36665
41 36665
42 36665
43 36665
44 36665
45 36665
46 36665
47 36665
48 36665
49 36665
50 36665
51 36665
52 36665
53 36665
54 36665
55 36665
56 36665
57 36665
58 36665
59 36665
60 36665
61 36665
62 36665
63 36665
64 36665
65 36665
66 36665
67 36665
68 36665
69 36665
70 36665
71 36665
72 36665
73 36665
74 36665
75 36665
76 36665
77 36665
78 36665
79 36665
80 36665
81 36665
82 36665
83 36665
84 36665
85 36665
86 36665
87 36665
88 36665
89 36665
90 36665
91 36665
92 36665
93 36665
94 36665
95 36665
96 36665
97 36665
98 36665
99 36665
};
\addplot [densely dotted, thick, forestgreen4416044]
table {%
1 10397.0
2 19671.0
3 25743.0
4 28807.0
5 30697.0
6 31913.0
7 32773.0
8 33414.0
9 33912.0
10 34298.0
11 34613.0
12 34876.0
13 35098.0
14 35282.0
15 35431.0
16 35555.0
17 35658.0
18 35744.0
19 35818.0
20 35883.0
21 35941.0
22 35989.0
23 36031.0
24 36069.0
25 36106.0
26 36139.0
27 36168.0
28 36192.0
29 36214.0
30 36235.0
31 36252.0
32 36267.0
33 36280.0
34 36293.0
35 36305.0
36 36315.0
37 36324.0
38 36333.0
39 36342.0
40 36350.0
41 36357.0
42 36364.0
43 36370.0
44 36376.0
45 36382.0
46 36388.0
47 36394.0
48 36400.0
49 36405.0
50 36410.0
51 36415.0
52 36420.0
53 36425.0
54 36430.0
55 36435.0
56 36440.0
57 36445.0
58 36450.0
59 36454.0
60 36458.0
61 36462.0
62 36466.0
63 36470.0
64 36474.0
65 36478.0
66 36482.0
67 36486.0
68 36490.0
69 36494.0
70 36498.0
71 36502.0
72 36506.0
73 36510.0
74 36514.0
75 36518.0
76 36522.0
77 36526.0
78 36530.0
79 36534.0
80 36538.0
81 36542.0
82 36546.0
83 36550.0
84 36554.0
85 36557.0
86 36560.0
87 36563.0
88 36566.0
89 36569.0
90 36572.0
91 36575.0
92 36578.0
93 36581.0
94 36584.0
95 36586.0
96 36588.0
97 36590.0
98 36592.0
99 36594.0
};
\addplot [densely dotted, thick, darkorange25512714]
table {%
1 9662.0
2 17182.0
3 22419.0
4 25877.0
5 28241.0
6 29895.0
7 31111.0
8 32043.0
9 32754.0
10 33328.0
11 33795.0
12 34187.0
13 34506.0
14 34761.0
15 34983.0
16 35173.0
17 35328.0
18 35459.0
19 35575.0
20 35674.0
21 35752.0
22 35823.0
23 35886.0
24 35940.0
25 35987.0
26 36029.0
27 36068.0
28 36103.0
29 36135.0
30 36164.0
31 36189.0
32 36212.0
33 36234.0
34 36253.0
35 36270.0
36 36285.0
37 36297.0
38 36308.0
39 36318.0
40 36327.0
41 36335.0
42 36343.0
43 36350.0
44 36357.0
45 36363.0
46 36369.0
47 36375.0
48 36381.0
49 36387.0
50 36393.0
51 36399.0
52 36405.0
53 36411.0
54 36416.0
55 36421.0
56 36426.0
57 36431.0
58 36436.0
59 36441.0
60 36446.0
61 36451.0
62 36456.0
63 36461.0
64 36466.0
65 36471.0
66 36476.0
67 36480.0
68 36484.0
69 36488.0
70 36492.0
71 36496.0
72 36500.0
73 36504.0
74 36508.0
75 36512.0
76 36516.0
77 36520.0
78 36524.0
79 36528.0
80 36532.0
81 36536.0
82 36540.0
83 36544.0
84 36548.0
85 36552.0
86 36556.0
87 36559.0
88 36562.0
89 36565.0
90 36568.0
91 36571.0
92 36574.0
93 36577.0
94 36580.0
95 36583.0
96 36586.0
97 36588.0
98 36590.0
99 36592.0
};
\path [fill=crimson2143940, fill opacity=0.2]
(axis cs:1,2779.8)--
(axis cs:1,2858.2)--
(axis cs:2,4221.1)--
(axis cs:3,5260.2)--
(axis cs:4,6108.0)--
(axis cs:5,6860.0)--
(axis cs:6,7492.4)--
(axis cs:7,8084.1)--
(axis cs:8,8636.0)--
(axis cs:9,9125.2)--
(axis cs:10,9591.5)--
(axis cs:11,10009.1)--
(axis cs:12,10460.2)--
(axis cs:13,10853.8)--
(axis cs:14,11223.4)--
(axis cs:15,11606.1)--
(axis cs:16,11949.3)--
(axis cs:17,12283.4)--
(axis cs:18,12591.6)--
(axis cs:19,12905.0)--
(axis cs:20,13219.3)--
(axis cs:21,13500.1)--
(axis cs:22,13799.0)--
(axis cs:23,14068.3)--
(axis cs:24,14327.4)--
(axis cs:25,14591.1)--
(axis cs:26,14838.4)--
(axis cs:27,15084.2)--
(axis cs:28,15318.8)--
(axis cs:29,15558.6)--
(axis cs:30,15786.1)--
(axis cs:31,16003.5)--
(axis cs:32,16226.7)--
(axis cs:33,16441.4)--
(axis cs:34,16660.3)--
(axis cs:35,16845.1)--
(axis cs:36,17045.3)--
(axis cs:37,17248.1)--
(axis cs:38,17455.3)--
(axis cs:39,17643.1)--
(axis cs:40,17838.1)--
(axis cs:41,18003.1)--
(axis cs:42,18189.1)--
(axis cs:43,18349.4)--
(axis cs:44,18506.0)--
(axis cs:45,18716.5)--
(axis cs:46,18876.7)--
(axis cs:47,19035.2)--
(axis cs:48,19199.2)--
(axis cs:49,19366.6)--
(axis cs:50,19510.7)--
(axis cs:51,19660.0)--
(axis cs:52,19832.1)--
(axis cs:53,19978.2)--
(axis cs:54,20114.4)--
(axis cs:55,20251.0)--
(axis cs:56,20398.7)--
(axis cs:57,20550.2)--
(axis cs:58,20689.2)--
(axis cs:59,20844.4)--
(axis cs:60,20961.2)--
(axis cs:61,21101.1)--
(axis cs:62,21242.3)--
(axis cs:63,21381.0)--
(axis cs:64,21509.1)--
(axis cs:65,21617.3)--
(axis cs:66,21729.3)--
(axis cs:67,21876.8)--
(axis cs:68,21986.6)--
(axis cs:69,22112.0)--
(axis cs:70,22227.4)--
(axis cs:71,22366.1)--
(axis cs:72,22457.4)--
(axis cs:73,22590.1)--
(axis cs:74,22716.4)--
(axis cs:75,22786.0)--
(axis cs:76,22911.1)--
(axis cs:77,23041.3)--
(axis cs:78,23135.4)--
(axis cs:79,23235.2)--
(axis cs:80,23339.3)--
(axis cs:81,23434.2)--
(axis cs:82,23530.6)--
(axis cs:83,23652.2)--
(axis cs:84,23756.1)--
(axis cs:85,23858.6)--
(axis cs:86,23948.2)--
(axis cs:87,24028.6)--
(axis cs:88,24160.0)--
(axis cs:89,24243.1)--
(axis cs:90,24345.3)--
(axis cs:91,24405.1)--
(axis cs:92,24503.0)--
(axis cs:93,24598.6)--
(axis cs:94,24691.2)--
(axis cs:95,24779.7)--
(axis cs:96,24877.1)--
(axis cs:97,24944.4)--
(axis cs:98,25040.8)--
(axis cs:99,25130.0)--
(axis cs:99,24966.8)--
(axis cs:98,24886.9)--
(axis cs:97,24802.1)--
(axis cs:96,24721.9)--
(axis cs:95,24638.6)--
(axis cs:94,24550.8)--
(axis cs:93,24445.9)--
(axis cs:92,24395.2)--
(axis cs:91,24243.8)--
(axis cs:90,24184.9)--
(axis cs:89,24075.5)--
(axis cs:88,23991.8)--
(axis cs:87,23879.9)--
(axis cs:86,23783.0)--
(axis cs:85,23714.2)--
(axis cs:84,23594.9)--
(axis cs:83,23491.7)--
(axis cs:82,23399.7)--
(axis cs:81,23286.6)--
(axis cs:80,23170.0)--
(axis cs:79,23080.5)--
(axis cs:78,22958.7)--
(axis cs:77,22854.8)--
(axis cs:76,22753.8)--
(axis cs:75,22634.7)--
(axis cs:74,22517.8)--
(axis cs:73,22433.0)--
(axis cs:72,22302.6)--
(axis cs:71,22190.3)--
(axis cs:70,22070.6)--
(axis cs:69,21951.4)--
(axis cs:68,21838.3)--
(axis cs:67,21701.4)--
(axis cs:66,21585.5)--
(axis cs:65,21452.0)--
(axis cs:64,21328.9)--
(axis cs:63,21185.9)--
(axis cs:62,21097.7)--
(axis cs:61,20943.9)--
(axis cs:60,20811.0)--
(axis cs:59,20694.2)--
(axis cs:58,20522.3)--
(axis cs:57,20393.0)--
(axis cs:56,20254.9)--
(axis cs:55,20129.9)--
(axis cs:54,19969.2)--
(axis cs:53,19804.8)--
(axis cs:52,19684.9)--
(axis cs:51,19502.2)--
(axis cs:50,19351.9)--
(axis cs:49,19210.2)--
(axis cs:48,19042.7)--
(axis cs:47,18869.5)--
(axis cs:46,18711.2)--
(axis cs:45,18532.3)--
(axis cs:44,18361.6)--
(axis cs:43,18204.9)--
(axis cs:42,18006.8)--
(axis cs:41,17841.8)--
(axis cs:40,17675.8)--
(axis cs:39,17479.8)--
(axis cs:38,17290.4)--
(axis cs:37,17073.9)--
(axis cs:36,16910.9)--
(axis cs:35,16680.9)--
(axis cs:34,16513.9)--
(axis cs:33,16270.4)--
(axis cs:32,16075.6)--
(axis cs:31,15858.3)--
(axis cs:30,15628.7)--
(axis cs:29,15386.2)--
(axis cs:28,15158.8)--
(axis cs:27,14929.3)--
(axis cs:26,14688.7)--
(axis cs:25,14424.8)--
(axis cs:24,14172.9)--
(axis cs:23,13903.6)--
(axis cs:22,13628.8)--
(axis cs:21,13346.2)--
(axis cs:20,13067.9)--
(axis cs:19,12758.8)--
(axis cs:18,12445.9)--
(axis cs:17,12153.9)--
(axis cs:16,11784.9)--
(axis cs:15,11455.6)--
(axis cs:14,11085.8)--
(axis cs:13,10702.7)--
(axis cs:12,10318.6)--
(axis cs:11,9890.0)--
(axis cs:10,9434.0)--
(axis cs:9,8970.9)--
(axis cs:8,8493.9)--
(axis cs:7,7944.0)--
(axis cs:6,7369.9)--
(axis cs:5,6724.5)--
(axis cs:4,5981.8)--
(axis cs:3,5144.9)--
(axis cs:2,4124.0)--
(axis cs:1,2779.8)--
cycle;
\addplot [dashdotted, thick, crimson2143940]
table {%
1 2813.0
2 4176.0
3 5207.5
4 6043.5
5 6784.0
6 7430.5
7 8006.5
8 8573.0
9 9061.5
10 9514.0
11 9954.5
12 10383.0
13 10778.0
14 11166.0
15 11534.0
16 11868.0
17 12210.0
18 12527.0
19 12836.0
20 13133.0
21 13432.0
22 13706.0
23 13991.0
24 14245.5
25 14497.0
26 14763.5
27 15006.5
28 15243.5
29 15475.5
30 15708.0
31 15932.5
32 16147.5
33 16370.0
34 16578.0
35 16770.5
36 16982.0
37 17175.5
38 17367.5
39 17565.0
40 17755.0
41 17924.5
42 18091.0
43 18289.5
44 18437.0
45 18641.5
46 18793.0
47 18957.5
48 19124.5
49 19286.5
50 19435.5
51 19581.0
52 19751.5
53 19895.0
54 20050.5
55 20193.0
56 20334.0
57 20467.5
58 20612.0
59 20768.5
60 20877.0
61 21020.5
62 21166.0
63 21296.5
64 21424.5
65 21552.0
66 21668.0
67 21794.5
68 21922.5
69 22035.0
70 22137.5
71 22278.5
72 22375.0
73 22506.0
74 22618.5
75 22719.5
76 22834.0
77 22944.5
78 23051.0
79 23169.0
80 23249.0
81 23362.5
82 23470.0
83 23570.0
84 23688.0
85 23779.0
86 23858.5
87 23949.5
88 24071.5
89 24152.0
90 24259.0
91 24318.5
92 24450.0
93 24515.5
94 24621.5
95 24697.5
96 24796.0
97 24867.0
98 24972.5
99 25053.5
};
\path [fill=darkgray176, fill opacity=0.2]
(axis cs:1,2756.9)--
(axis cs:1,2857.2)--
(axis cs:2,7853.9)--
(axis cs:3,13389.4)--
(axis cs:4,18431.6)--
(axis cs:5,22521.3)--
(axis cs:6,25592.3)--
(axis cs:7,27866.3)--
(axis cs:8,29571.5)--
(axis cs:9,30859.3)--
(axis cs:10,31830.0)--
(axis cs:11,32563.1)--
(axis cs:12,33164.1)--
(axis cs:13,33641.5)--
(axis cs:14,34032.3)--
(axis cs:15,34369.0)--
(axis cs:16,34641.1)--
(axis cs:17,34881.1)--
(axis cs:18,35081.1)--
(axis cs:19,35254.0)--
(axis cs:20,35396.0)--
(axis cs:21,35521.1)--
(axis cs:22,35628.1)--
(axis cs:23,35719.0)--
(axis cs:24,35792.1)--
(axis cs:25,35863.0)--
(axis cs:26,35920.0)--
(axis cs:27,35971.0)--
(axis cs:28,36012.1)--
(axis cs:29,36058.0)--
(axis cs:30,36091.2)--
(axis cs:31,36126.1)--
(axis cs:32,36154.1)--
(axis cs:33,36182.0)--
(axis cs:34,36206.0)--
(axis cs:35,36227.0)--
(axis cs:36,36244.0)--
(axis cs:37,36263.0)--
(axis cs:38,36277.1)--
(axis cs:39,36293.1)--
(axis cs:40,36305.1)--
(axis cs:41,36317.0)--
(axis cs:42,36326.0)--
(axis cs:43,36336.0)--
(axis cs:44,36343.0)--
(axis cs:45,36352.0)--
(axis cs:46,36358.0)--
(axis cs:47,36366.0)--
(axis cs:48,36372.1)--
(axis cs:49,36379.0)--
(axis cs:50,36384.1)--
(axis cs:51,36389.1)--
(axis cs:52,36395.1)--
(axis cs:53,36402.0)--
(axis cs:54,36408.0)--
(axis cs:55,36414.0)--
(axis cs:56,36420.0)--
(axis cs:57,36425.0)--
(axis cs:58,36431.0)--
(axis cs:59,36434.1)--
(axis cs:60,36440.0)--
(axis cs:61,36445.0)--
(axis cs:62,36450.0)--
(axis cs:63,36455.0)--
(axis cs:64,36458.0)--
(axis cs:65,36463.0)--
(axis cs:66,36468.0)--
(axis cs:67,36472.0)--
(axis cs:68,36476.0)--
(axis cs:69,36481.0)--
(axis cs:70,36484.0)--
(axis cs:71,36488.0)--
(axis cs:72,36492.1)--
(axis cs:73,36496.0)--
(axis cs:74,36500.0)--
(axis cs:75,36503.1)--
(axis cs:76,36509.0)--
(axis cs:77,36512.0)--
(axis cs:78,36516.0)--
(axis cs:79,36519.0)--
(axis cs:80,36523.0)--
(axis cs:81,36528.0)--
(axis cs:82,36532.0)--
(axis cs:83,36537.0)--
(axis cs:84,36541.0)--
(axis cs:85,36544.0)--
(axis cs:86,36548.0)--
(axis cs:87,36551.0)--
(axis cs:88,36555.1)--
(axis cs:89,36559.0)--
(axis cs:90,36562.0)--
(axis cs:91,36566.0)--
(axis cs:92,36568.1)--
(axis cs:93,36571.0)--
(axis cs:94,36575.0)--
(axis cs:95,36577.1)--
(axis cs:96,36581.0)--
(axis cs:97,36584.0)--
(axis cs:98,36586.0)--
(axis cs:99,36589.0)--
(axis cs:99,36584.0)--
(axis cs:98,36580.0)--
(axis cs:97,36577.0)--
(axis cs:96,36575.0)--
(axis cs:95,36571.0)--
(axis cs:94,36569.0)--
(axis cs:93,36565.9)--
(axis cs:92,36563.0)--
(axis cs:91,36560.0)--
(axis cs:90,36556.0)--
(axis cs:89,36552.9)--
(axis cs:88,36549.0)--
(axis cs:87,36545.0)--
(axis cs:86,36541.9)--
(axis cs:85,36537.0)--
(axis cs:84,36533.0)--
(axis cs:83,36529.9)--
(axis cs:82,36525.0)--
(axis cs:81,36522.0)--
(axis cs:80,36517.0)--
(axis cs:79,36513.0)--
(axis cs:78,36509.9)--
(axis cs:77,36505.0)--
(axis cs:76,36501.0)--
(axis cs:75,36496.0)--
(axis cs:74,36494.0)--
(axis cs:73,36489.0)--
(axis cs:72,36484.9)--
(axis cs:71,36481.0)--
(axis cs:70,36476.0)--
(axis cs:69,36473.0)--
(axis cs:68,36470.0)--
(axis cs:67,36465.0)--
(axis cs:66,36461.0)--
(axis cs:65,36456.0)--
(axis cs:64,36452.0)--
(axis cs:63,36446.9)--
(axis cs:62,36443.0)--
(axis cs:61,36438.0)--
(axis cs:60,36433.0)--
(axis cs:59,36426.0)--
(axis cs:58,36423.0)--
(axis cs:57,36416.0)--
(axis cs:56,36412.0)--
(axis cs:55,36406.0)--
(axis cs:54,36400.0)--
(axis cs:53,36393.0)--
(axis cs:52,36388.0)--
(axis cs:51,36382.0)--
(axis cs:50,36376.0)--
(axis cs:49,36369.0)--
(axis cs:48,36363.0)--
(axis cs:47,36357.0)--
(axis cs:46,36349.0)--
(axis cs:45,36342.0)--
(axis cs:44,36332.0)--
(axis cs:43,36324.0)--
(axis cs:42,36315.0)--
(axis cs:41,36305.0)--
(axis cs:40,36293.0)--
(axis cs:39,36280.9)--
(axis cs:38,36265.9)--
(axis cs:37,36247.0)--
(axis cs:36,36228.0)--
(axis cs:35,36210.0)--
(axis cs:34,36189.9)--
(axis cs:33,36167.0)--
(axis cs:32,36139.0)--
(axis cs:31,36106.0)--
(axis cs:30,36070.8)--
(axis cs:29,36035.7)--
(axis cs:28,35991.9)--
(axis cs:27,35947.9)--
(axis cs:26,35896.9)--
(axis cs:25,35836.0)--
(axis cs:24,35767.9)--
(axis cs:23,35692.9)--
(axis cs:22,35597.0)--
(axis cs:21,35490.9)--
(axis cs:20,35365.9)--
(axis cs:19,35215.9)--
(axis cs:18,35040.0)--
(axis cs:17,34841.9)--
(axis cs:16,34597.0)--
(axis cs:15,34321.0)--
(axis cs:14,33986.9)--
(axis cs:13,33592.9)--
(axis cs:12,33098.9)--
(axis cs:11,32503.7)--
(axis cs:10,31752.9)--
(axis cs:9,30763.9)--
(axis cs:8,29492.8)--
(axis cs:7,27761.0)--
(axis cs:6,25470.0)--
(axis cs:5,22367.2)--
(axis cs:4,18272.7)--
(axis cs:3,13221.2)--
(axis cs:2,7722.9)--
(axis cs:1,2756.9)--
cycle;
% \addplot [thick, darkgray176]
% table {%
% 1 2807.5
% 2 7790.0
% 3 13308.5
% 4 18346.0
% 5 22449.0
% 6 25537.5
% 7 27819.0
% 8 29528.5
% 9 30818.5
% 10 31789.0
% 11 32535.0
% 12 33132.5
% 13 33617.0
% 14 34012.5
% 15 34344.0
% 16 34618.0
% 17 34862.5
% 18 35060.0
% 19 35236.5
% 20 35381.0
% 21 35504.5
% 22 35611.0
% 23 35704.0
% 24 35780.0
% 25 35848.0
% 26 35907.0
% 27 35958.0
% 28 36005.0
% 29 36045.0
% 30 36082.0
% 31 36117.0
% 32 36146.0
% 33 36175.0
% 34 36198.0
% 35 36218.0
% 36 36237.0
% 37 36256.0
% 38 36272.5
% 39 36286.0
% 40 36299.0
% 41 36311.0
% 42 36321.0
% 43 36330.0
% 44 36339.0
% 45 36346.0
% 46 36354.0
% 47 36361.0
% 48 36367.5
% 49 36374.0
% 50 36380.0
% 51 36386.0
% 52 36392.0
% 53 36397.0
% 54 36404.0
% 55 36410.0
% 56 36415.5
% 57 36420.0
% 58 36426.0
% 59 36431.0
% 60 36436.0
% 61 36441.0
% 62 36446.0
% 63 36451.0
% 64 36455.0
% 65 36460.0
% 66 36464.5
% 67 36468.5
% 68 36473.0
% 69 36477.0
% 70 36480.0
% 71 36485.0
% 72 36489.0
% 73 36492.0
% 74 36497.0
% 75 36501.0
% 76 36505.0
% 77 36509.0
% 78 36513.0
% 79 36516.0
% 80 36520.0
% 81 36525.0
% 82 36529.0
% 83 36533.0
% 84 36537.0
% 85 36540.0
% 86 36545.0
% 87 36548.0
% 88 36552.5
% 89 36556.0
% 90 36559.0
% 91 36563.0
% 92 36565.0
% 93 36569.0
% 94 36572.0
% 95 36575.0
% 96 36578.0
% 97 36581.0
% 98 36584.0
% 99 36586.0
% };


==> figures/bounds/askreddit.tex <==
\nextgroupplot [
    title=Reddit,
    xmin=-0.4, xmax=103.9,
    ymin=18533.755, ymax=106849.345,
    ylabel={Distinct Count},
]
\addplot [dashed, steelblue31119180]
table {%
1 102835
2 102835
3 102835
4 102835
5 102835
6 102835
7 102835
8 102835
9 102835
10 102835
11 102835
12 102835
13 102835
14 102835
15 102835
16 102835
17 102835
18 102835
19 102835
20 102835
21 102835
22 102835
23 102835
24 102835
25 102835
26 102835
27 102835
28 102835
29 102835
30 102835
31 102835
32 102835
33 102835
34 102835
35 102835
36 102835
37 102835
38 102835
39 102835
40 102835
41 102835
42 102835
43 102835
44 102835
45 102835
46 102835
47 102835
48 102835
49 102835
50 102835
51 102835
52 102835
53 102835
54 102835
55 102835
56 102835
57 102835
58 102835
59 102835
60 102835
61 102835
62 102835
63 102835
64 102835
65 102835
66 102835
67 102835
68 102835
69 102835
70 102835
71 102835
72 102835
73 102835
74 102835
75 102835
76 102835
77 102835
78 102835
79 102835
80 102835
81 102835
82 102835
83 102835
84 102835
85 102835
86 102835
87 102835
88 102835
89 102835
90 102835
91 102835
92 102835
93 102835
94 102835
95 102835
96 102835
97 102835
98 102835
99 102835
};
\addplot [densely dotted, thick, forestgreen4416044]
table {%
1 82929.0
2 94356.0
3 98067.0
4 99687.0
5 100552.0
6 101076.0
7 101439.0
8 101702.0
9 101891.0
10 102030.0
11 102141.0
12 102232.0
13 102302.0
14 102357.0
15 102400.0
16 102436.0
17 102465.0
18 102490.0
19 102513.0
20 102534.0
21 102555.0
22 102573.0
23 102591.0
24 102608.0
25 102623.0
26 102636.0
27 102646.0
28 102656.0
29 102664.0
30 102671.0
31 102678.0
32 102685.0
33 102691.0
34 102697.0
35 102703.0
36 102709.0
37 102715.0
38 102721.0
39 102726.0
40 102730.0
41 102734.0
42 102738.0
43 102742.0
44 102746.0
45 102749.0
46 102752.0
47 102755.0
48 102758.0
49 102761.0
50 102763.0
51 102765.0
52 102767.0
53 102769.0
54 102771.0
55 102773.0
56 102775.0
57 102777.0
58 102779.0
59 102781.0
60 102783.0
61 102785.0
62 102786.0
63 102787.0
64 102788.0
65 102789.0
66 102790.0
67 102791.0
68 102792.0
69 102793.0
70 102794.0
71 102795.0
72 102796.0
73 102797.0
74 102798.0
75 102799.0
76 102800.0
77 102801.0
78 102802.0
79 102803.0
80 102804.0
81 102805.0
82 102806.0
83 102807.0
84 102808.0
85 102809.0
86 102810.0
87 102811.0
88 102812.0
89 102813.0
90 102814.0
91 102815.0
92 102816.0
93 102817.0
94 102818.0
95 102819.0
96 102820.0
97 102821.0
98 102822.0
99 102823.0
};
\addplot [densely dotted, thick, darkorange25512714]
table {%
1 73161.0
2 90093.0
3 95996.0
4 98570.0
5 99885.0
6 100636.0
7 101116.0
8 101469.0
9 101721.0
10 101903.0
11 102033.0
12 102139.0
13 102230.0
14 102301.0
15 102358.0
16 102401.0
17 102435.0
18 102465.0
19 102491.0
20 102516.0
21 102538.0
22 102558.0
23 102577.0
24 102594.0
25 102610.0
26 102624.0
27 102636.0
28 102647.0
29 102657.0
30 102664.0
31 102671.0
32 102678.0
33 102685.0
34 102691.0
35 102697.0
36 102703.0
37 102709.0
38 102715.0
39 102721.0
40 102725.0
41 102729.0
42 102733.0
43 102737.0
44 102741.0
45 102744.0
46 102747.0
47 102750.0
48 102753.0
49 102756.0
50 102759.0
51 102762.0
52 102764.0
53 102766.0
54 102768.0
55 102770.0
56 102772.0
57 102774.0
58 102776.0
59 102778.0
60 102780.0
61 102782.0
62 102784.0
63 102785.0
64 102786.0
65 102787.0
66 102788.0
67 102789.0
68 102790.0
69 102791.0
70 102792.0
71 102793.0
72 102794.0
73 102795.0
74 102796.0
75 102797.0
76 102798.0
77 102799.0
78 102800.0
79 102801.0
80 102802.0
81 102803.0
82 102804.0
83 102805.0
84 102806.0
85 102807.0
86 102808.0
87 102809.0
88 102810.0
89 102811.0
90 102812.0
91 102813.0
92 102814.0
93 102815.0
94 102816.0
95 102817.0
96 102818.0
97 102819.0
98 102820.0
99 102821.0
};
\path [fill=crimson2143940, fill opacity=0.2]
(axis cs:1,22547.0)--
(axis cs:1,22734.0)--
(axis cs:2,31389.5)--
(axis cs:3,37230.1)--
(axis cs:4,41772.2)--
(axis cs:5,45497.1)--
(axis cs:6,48672.4)--
(axis cs:7,51399.5)--
(axis cs:8,53837.2)--
(axis cs:9,56034.2)--
(axis cs:10,58009.4)--
(axis cs:11,59809.7)--
(axis cs:12,61460.8)--
(axis cs:13,63005.1)--
(axis cs:14,64427.0)--
(axis cs:15,65725.6)--
(axis cs:16,67014.6)--
(axis cs:17,68179.1)--
(axis cs:18,69238.4)--
(axis cs:19,70277.3)--
(axis cs:20,71288.1)--
(axis cs:21,72206.6)--
(axis cs:22,73060.2)--
(axis cs:23,73906.0)--
(axis cs:24,74691.6)--
(axis cs:25,75463.1)--
(axis cs:26,76198.7)--
(axis cs:27,76868.2)--
(axis cs:28,77543.9)--
(axis cs:29,78169.1)--
(axis cs:30,78771.1)--
(axis cs:31,79362.1)--
(axis cs:32,79905.4)--
(axis cs:33,80437.6)--
(axis cs:34,80979.2)--
(axis cs:35,81470.2)--
(axis cs:36,81975.1)--
(axis cs:37,82426.2)--
(axis cs:38,82890.7)--
(axis cs:39,83312.9)--
(axis cs:40,83726.2)--
(axis cs:41,84116.0)--
(axis cs:42,84503.4)--
(axis cs:43,84892.1)--
(axis cs:44,85253.1)--
(axis cs:45,85629.1)--
(axis cs:46,85974.1)--
(axis cs:47,86306.4)--
(axis cs:48,86643.1)--
(axis cs:49,86936.3)--
(axis cs:50,87253.7)--
(axis cs:51,87538.7)--
(axis cs:52,87858.2)--
(axis cs:53,88109.7)--
(axis cs:54,88371.2)--
(axis cs:55,88653.1)--
(axis cs:56,88910.3)--
(axis cs:57,89158.0)--
(axis cs:58,89412.6)--
(axis cs:59,89652.1)--
(axis cs:60,89880.0)--
(axis cs:61,90126.0)--
(axis cs:62,90324.0)--
(axis cs:63,90523.6)--
(axis cs:64,90744.4)--
(axis cs:65,90945.0)--
(axis cs:66,91168.0)--
(axis cs:67,91369.2)--
(axis cs:68,91547.2)--
(axis cs:69,91724.4)--
(axis cs:70,91903.1)--
(axis cs:71,92083.0)--
(axis cs:72,92271.0)--
(axis cs:73,92420.3)--
(axis cs:74,92594.0)--
(axis cs:75,92768.3)--
(axis cs:76,92924.1)--
(axis cs:77,93063.2)--
(axis cs:78,93219.2)--
(axis cs:79,93365.7)--
(axis cs:80,93504.2)--
(axis cs:81,93638.0)--
(axis cs:82,93795.5)--
(axis cs:83,93907.1)--
(axis cs:84,94051.6)--
(axis cs:85,94187.0)--
(axis cs:86,94303.5)--
(axis cs:87,94425.8)--
(axis cs:88,94547.3)--
(axis cs:89,94683.1)--
(axis cs:90,94788.2)--
(axis cs:91,94901.0)--
(axis cs:92,95028.5)--
(axis cs:93,95137.2)--
(axis cs:94,95249.2)--
(axis cs:95,95355.0)--
(axis cs:96,95470.1)--
(axis cs:97,95545.0)--
(axis cs:98,95664.9)--
(axis cs:99,95748.0)--
(axis cs:99,95611.9)--
(axis cs:98,95512.6)--
(axis cs:97,95401.3)--
(axis cs:96,95310.6)--
(axis cs:95,95213.3)--
(axis cs:94,95078.9)--
(axis cs:93,94976.6)--
(axis cs:92,94880.9)--
(axis cs:91,94751.7)--
(axis cs:90,94643.9)--
(axis cs:89,94526.5)--
(axis cs:88,94403.8)--
(axis cs:87,94277.7)--
(axis cs:86,94170.7)--
(axis cs:85,94034.0)--
(axis cs:84,93892.0)--
(axis cs:83,93755.0)--
(axis cs:82,93634.0)--
(axis cs:81,93474.9)--
(axis cs:80,93345.9)--
(axis cs:79,93215.3)--
(axis cs:78,93063.1)--
(axis cs:77,92902.9)--
(axis cs:76,92747.6)--
(axis cs:75,92595.6)--
(axis cs:74,92425.3)--
(axis cs:73,92262.0)--
(axis cs:72,92081.5)--
(axis cs:71,91925.9)--
(axis cs:70,91734.7)--
(axis cs:69,91560.9)--
(axis cs:68,91391.7)--
(axis cs:67,91197.6)--
(axis cs:66,90978.9)--
(axis cs:65,90773.5)--
(axis cs:64,90579.0)--
(axis cs:63,90370.5)--
(axis cs:62,90142.9)--
(axis cs:61,89946.7)--
(axis cs:60,89707.7)--
(axis cs:59,89481.8)--
(axis cs:58,89210.0)--
(axis cs:57,89004.4)--
(axis cs:56,88714.9)--
(axis cs:55,88476.6)--
(axis cs:54,88198.8)--
(axis cs:53,87929.8)--
(axis cs:52,87660.6)--
(axis cs:51,87357.2)--
(axis cs:50,87065.8)--
(axis cs:49,86749.2)--
(axis cs:48,86435.6)--
(axis cs:47,86110.9)--
(axis cs:46,85788.6)--
(axis cs:45,85440.8)--
(axis cs:44,85067.2)--
(axis cs:43,84708.3)--
(axis cs:42,84345.4)--
(axis cs:41,83951.6)--
(axis cs:40,83513.4)--
(axis cs:39,83098.5)--
(axis cs:38,82658.2)--
(axis cs:37,82219.6)--
(axis cs:36,81765.0)--
(axis cs:35,81258.1)--
(axis cs:34,80787.1)--
(axis cs:33,80247.9)--
(axis cs:32,79672.8)--
(axis cs:31,79118.8)--
(axis cs:30,78552.8)--
(axis cs:29,77951.7)--
(axis cs:28,77302.9)--
(axis cs:27,76644.7)--
(axis cs:26,75942.9)--
(axis cs:25,75221.8)--
(axis cs:24,74468.3)--
(axis cs:23,73669.8)--
(axis cs:22,72845.7)--
(axis cs:21,71969.0)--
(axis cs:20,71037.0)--
(axis cs:19,70049.4)--
(axis cs:18,68984.5)--
(axis cs:17,67917.9)--
(axis cs:16,66757.8)--
(axis cs:15,65513.5)--
(axis cs:14,64165.8)--
(axis cs:13,62739.7)--
(axis cs:12,61222.4)--
(axis cs:11,59539.2)--
(axis cs:10,57750.8)--
(axis cs:9,55744.8)--
(axis cs:8,53575.0)--
(axis cs:7,51161.3)--
(axis cs:6,48409.6)--
(axis cs:5,45257.5)--
(axis cs:4,41535.6)--
(axis cs:3,37012.2)--
(axis cs:2,31159.1)--
(axis cs:1,22547.0)--
cycle;
\addplot [dashdotted, thick, crimson2143940]
table {%
1 22632.0
2 31255.0
3 37119.0
4 41646.5
5 45390.0
6 48535.0
7 51277.0
8 53706.0
9 55876.5
10 57881.0
11 59661.0
12 61347.0
13 62884.5
14 64303.0
15 65617.5
16 66872.5
17 68042.0
18 69122.0
19 70167.5
20 71157.5
21 72070.0
22 72961.5
23 73801.0
24 74574.5
25 75330.5
26 76061.0
27 76743.5
28 77416.5
29 78052.0
30 78656.5
31 79252.5
32 79807.5
33 80362.5
34 80880.0
35 81371.5
36 81878.5
37 82301.0
38 82794.5
39 83224.5
40 83620.0
41 84043.5
42 84427.5
43 84794.0
44 85162.0
45 85517.5
46 85876.5
47 86213.0
48 86521.0
49 86849.0
50 87149.0
51 87442.0
52 87735.0
53 88022.5
54 88305.0
55 88557.5
56 88822.0
57 89074.0
58 89310.5
59 89562.0
60 89802.5
61 90034.5
62 90244.0
63 90449.5
64 90657.5
65 90868.5
66 91078.5
67 91272.5
68 91464.5
69 91635.5
70 91821.5
71 92002.5
72 92175.0
73 92341.5
74 92504.5
75 92671.5
76 92831.0
77 92991.0
78 93130.0
79 93279.0
80 93431.0
81 93560.0
82 93698.5
83 93843.0
84 93964.5
85 94114.0
86 94234.0
87 94359.0
88 94473.5
89 94604.0
90 94714.0
91 94834.0
92 94954.0
93 95055.5
94 95171.0
95 95281.5
96 95387.0
97 95481.5
98 95593.0
99 95677.0
};
\path [fill=darkgray176, fill opacity=0.2]
(axis cs:1,22522.0)--
(axis cs:1,22741.2)--
(axis cs:2,65210.0)--
(axis cs:3,87163.3)--
(axis cs:4,95016.3)--
(axis cs:5,98201.3)--
(axis cs:6,99737.0)--
(axis cs:7,100576.0)--
(axis cs:8,101098.1)--
(axis cs:9,101457.1)--
(axis cs:10,101717.0)--
(axis cs:11,101907.0)--
(axis cs:12,102044.0)--
(axis cs:13,102149.1)--
(axis cs:14,102240.0)--
(axis cs:15,102315.0)--
(axis cs:16,102369.1)--
(axis cs:17,102411.0)--
(axis cs:18,102445.0)--
(axis cs:19,102474.1)--
(axis cs:20,102499.0)--
(axis cs:21,102522.0)--
(axis cs:22,102544.0)--
(axis cs:23,102564.0)--
(axis cs:24,102581.1)--
(axis cs:25,102600.1)--
(axis cs:26,102615.0)--
(axis cs:27,102629.0)--
(axis cs:28,102642.0)--
(axis cs:29,102653.0)--
(axis cs:30,102662.0)--
(axis cs:31,102670.0)--
(axis cs:32,102677.0)--
(axis cs:33,102684.0)--
(axis cs:34,102690.0)--
(axis cs:35,102695.1)--
(axis cs:36,102702.0)--
(axis cs:37,102708.0)--
(axis cs:38,102714.0)--
(axis cs:39,102720.0)--
(axis cs:40,102726.0)--
(axis cs:41,102730.0)--
(axis cs:42,102734.0)--
(axis cs:43,102738.0)--
(axis cs:44,102742.0)--
(axis cs:45,102746.0)--
(axis cs:46,102749.0)--
(axis cs:47,102752.0)--
(axis cs:48,102755.0)--
(axis cs:49,102758.1)--
(axis cs:50,102761.0)--
(axis cs:51,102764.0)--
(axis cs:52,102766.0)--
(axis cs:53,102768.0)--
(axis cs:54,102770.0)--
(axis cs:55,102772.0)--
(axis cs:56,102774.0)--
(axis cs:57,102776.0)--
(axis cs:58,102778.0)--
(axis cs:59,102780.0)--
(axis cs:60,102782.0)--
(axis cs:61,102784.0)--
(axis cs:62,102785.1)--
(axis cs:63,102787.0)--
(axis cs:64,102788.0)--
(axis cs:65,102788.0)--
(axis cs:66,102790.0)--
(axis cs:67,102790.0)--
(axis cs:68,102792.0)--
(axis cs:69,102792.0)--
(axis cs:70,102794.0)--
(axis cs:71,102795.0)--
(axis cs:72,102796.0)--
(axis cs:73,102797.0)--
(axis cs:74,102798.0)--
(axis cs:75,102798.0)--
(axis cs:76,102800.0)--
(axis cs:77,102800.1)--
(axis cs:78,102802.0)--
(axis cs:79,102803.0)--
(axis cs:80,102803.0)--
(axis cs:81,102805.0)--
(axis cs:82,102806.0)--
(axis cs:83,102806.0)--
(axis cs:84,102808.0)--
(axis cs:85,102809.0)--
(axis cs:86,102810.0)--
(axis cs:87,102810.0)--
(axis cs:88,102811.1)--
(axis cs:89,102813.0)--
(axis cs:90,102814.0)--
(axis cs:91,102814.0)--
(axis cs:92,102816.0)--
(axis cs:93,102816.0)--
(axis cs:94,102818.0)--
(axis cs:95,102819.0)--
(axis cs:96,102819.1)--
(axis cs:97,102821.0)--
(axis cs:98,102822.0)--
(axis cs:99,102822.1)--
(axis cs:99,102821.0)--
(axis cs:98,102820.0)--
(axis cs:97,102819.0)--
(axis cs:96,102817.0)--
(axis cs:95,102816.9)--
(axis cs:94,102816.0)--
(axis cs:93,102814.0)--
(axis cs:92,102814.0)--
(axis cs:91,102812.0)--
(axis cs:90,102811.0)--
(axis cs:89,102810.9)--
(axis cs:88,102810.0)--
(axis cs:87,102808.0)--
(axis cs:86,102807.0)--
(axis cs:85,102806.9)--
(axis cs:84,102806.0)--
(axis cs:83,102804.0)--
(axis cs:82,102803.0)--
(axis cs:81,102803.0)--
(axis cs:80,102801.0)--
(axis cs:79,102801.0)--
(axis cs:78,102800.0)--
(axis cs:77,102799.0)--
(axis cs:76,102797.0)--
(axis cs:75,102797.0)--
(axis cs:74,102796.0)--
(axis cs:73,102794.0)--
(axis cs:72,102793.0)--
(axis cs:71,102792.0)--
(axis cs:70,102791.9)--
(axis cs:69,102791.0)--
(axis cs:68,102790.0)--
(axis cs:67,102789.0)--
(axis cs:66,102787.0)--
(axis cs:65,102787.0)--
(axis cs:64,102786.0)--
(axis cs:63,102784.0)--
(axis cs:62,102783.0)--
(axis cs:61,102781.0)--
(axis cs:60,102779.0)--
(axis cs:59,102777.0)--
(axis cs:58,102775.0)--
(axis cs:57,102773.0)--
(axis cs:56,102771.0)--
(axis cs:55,102769.0)--
(axis cs:54,102767.0)--
(axis cs:53,102765.0)--
(axis cs:52,102763.0)--
(axis cs:51,102760.0)--
(axis cs:50,102757.0)--
(axis cs:49,102754.0)--
(axis cs:48,102751.0)--
(axis cs:47,102748.0)--
(axis cs:46,102745.0)--
(axis cs:45,102742.0)--
(axis cs:44,102738.0)--
(axis cs:43,102734.0)--
(axis cs:42,102730.0)--
(axis cs:41,102726.0)--
(axis cs:40,102721.0)--
(axis cs:39,102716.0)--
(axis cs:38,102708.9)--
(axis cs:37,102703.0)--
(axis cs:36,102697.0)--
(axis cs:35,102690.9)--
(axis cs:34,102685.0)--
(axis cs:33,102679.0)--
(axis cs:32,102672.0)--
(axis cs:31,102664.0)--
(axis cs:30,102656.0)--
(axis cs:29,102646.0)--
(axis cs:28,102635.0)--
(axis cs:27,102621.9)--
(axis cs:26,102607.0)--
(axis cs:25,102591.0)--
(axis cs:24,102574.0)--
(axis cs:23,102555.0)--
(axis cs:22,102535.9)--
(axis cs:21,102512.9)--
(axis cs:20,102490.0)--
(axis cs:19,102464.0)--
(axis cs:18,102434.0)--
(axis cs:17,102399.0)--
(axis cs:16,102355.0)--
(axis cs:15,102299.0)--
(axis cs:14,102224.9)--
(axis cs:13,102132.9)--
(axis cs:12,102022.9)--
(axis cs:11,101880.9)--
(axis cs:10,101688.0)--
(axis cs:9,101426.9)--
(axis cs:8,101062.9)--
(axis cs:7,100535.9)--
(axis cs:6,99677.8)--
(axis cs:5,98137.9)--
(axis cs:4,94915.9)--
(axis cs:3,86987.0)--
(axis cs:2,64929.6)--
(axis cs:1,22522.0)--
cycle;
% \addplot [thick, darkgray176]
% table {%
% 1 22639.0
% 2 65073.5
% 3 87074.5
% 4 94966.0
% 5 98169.0
% 6 99704.0
% 7 100553.0
% 8 101079.5
% 9 101440.0
% 10 101702.5
% 11 101895.0
% 12 102033.0
% 13 102141.0
% 14 102233.0
% 15 102307.0
% 16 102363.0
% 17 102406.0
% 18 102440.0
% 19 102469.0
% 20 102494.0
% 21 102517.0
% 22 102540.0
% 23 102560.0
% 24 102578.0
% 25 102595.0
% 26 102611.0
% 27 102626.0
% 28 102639.0
% 29 102649.0
% 30 102659.0
% 31 102667.0
% 32 102674.0
% 33 102681.0
% 34 102687.0
% 35 102693.0
% 36 102699.0
% 37 102705.0
% 38 102712.0
% 39 102718.0
% 40 102723.0
% 41 102728.0
% 42 102732.0
% 43 102736.0
% 44 102740.0
% 45 102744.0
% 46 102747.0
% 47 102750.0
% 48 102753.0
% 49 102756.0
% 50 102759.0
% 51 102762.0
% 52 102764.5
% 53 102766.0
% 54 102768.0
% 55 102771.0
% 56 102772.0
% 57 102774.0
% 58 102777.0
% 59 102779.0
% 60 102781.0
% 61 102783.0
% 62 102784.0
% 63 102785.0
% 64 102786.5
% 65 102788.0
% 66 102789.0
% 67 102790.0
% 68 102791.0
% 69 102792.0
% 70 102793.0
% 71 102794.0
% 72 102795.0
% 73 102796.0
% 74 102797.0
% 75 102798.0
% 76 102799.0
% 77 102800.0
% 78 102801.0
% 79 102802.0
% 80 102802.0
% 81 102804.0
% 82 102804.0
% 83 102805.0
% 84 102807.0
% 85 102808.0
% 86 102809.0
% 87 102810.0
% 88 102811.0
% 89 102812.0
% 90 102812.0
% 91 102813.5
% 92 102815.0
% 93 102816.0
% 94 102817.0
% 95 102817.0
% 96 102819.0
% 97 102820.0
% 98 102821.0
% 99 102821.5
% };


==> figures/bounds/imdb.tex <==
\nextgroupplot [
    title=IMDB,
    xmin=-0.4, xmax=30.4,
    ymin=4893.8, ymax=103194.2,
]
\addplot [dashed, steelblue31119180]
table {%
1 98726
2 98726
3 98726
4 98726
5 98726
6 98726
7 98726
8 98726
9 98726
10 98726
11 98726
12 98726
13 98726
14 98726
15 98726
16 98726
17 98726
18 98726
19 98726
20 98726
21 98726
22 98726
23 98726
24 98726
25 98726
26 98726
27 98726
28 98726
29 98726
30 98726
31 98726
32 98726
33 98726
34 98726
35 98726
36 98726
37 98726
38 98726
39 98726
40 98726
41 98726
42 98726
43 98726
44 98726
45 98726
46 98726
47 98726
48 98726
49 98726
50 98726
51 98726
52 98726
53 98726
54 98726
55 98726
56 98726
57 98726
58 98726
59 98726
60 98726
61 98726
62 98726
63 98726
64 98726
65 98726
66 98726
67 98726
68 98726
69 98726
70 98726
71 98726
72 98726
73 98726
74 98726
75 98726
76 98726
77 98726
78 98726
79 98726
80 98726
81 98726
82 98726
83 98726
84 98726
85 98726
86 98726
87 98726
88 98726
89 98726
90 98726
91 98726
92 98726
93 98726
94 98726
95 98726
96 98726
97 98726
98 98726
99 98726
};
\addplot [densely dotted, thick, forestgreen4416044]
table {%
1 50000.0
2 82991.0
3 90667.0
4 94166.0
5 95946.0
6 96931.0
7 97547.0
8 97926.0
9 98187.0
10 98352.0
11 98456.0
12 98531.0
13 98586.0
14 98624.0
15 98653.0
16 98674.0
17 98690.0
18 98703.0
19 98712.0
20 98717.0
21 98721.0
22 98724.0
23 98726.0
24 98726.0
25 98726.0
26 98726.0
27 98726.0
28 98726.0
29 98726.0
30 98726.0
31 98726.0
32 98726.0
33 98726.0
34 98726.0
35 98726.0
36 98726.0
37 98726.0
38 98726.0
39 98726.0
40 98726.0
41 98726.0
42 98726.0
43 98726.0
44 98726.0
45 98726.0
46 98726.0
47 98726.0
48 98726.0
49 98726.0
50 98726.0
51 98726.0
52 98726.0
53 98726.0
54 98726.0
55 98726.0
56 98726.0
57 98726.0
58 98726.0
59 98726.0
60 98726.0
61 98726.0
62 98726.0
63 98726.0
64 98726.0
65 98726.0
66 98726.0
67 98726.0
68 98726.0
69 98726.0
70 98726.0
71 98726.0
72 98726.0
73 98726.0
74 98726.0
75 98726.0
76 98726.0
77 98726.0
78 98726.0
79 98726.0
80 98726.0
81 98726.0
82 98726.0
83 98726.0
84 98726.0
85 98726.0
86 98726.0
87 98726.0
88 98726.0
89 98726.0
90 98726.0
91 98726.0
92 98726.0
93 98726.0
94 98726.0
95 98726.0
96 98726.0
97 98726.0
98 98726.0
99 98726.0
};
\addplot [densely dotted, thick, darkorange25512714]
table {%
1 46454.0
2 72204.0
3 84007.0
4 90051.0
5 93372.0
6 95291.0
7 96440.0
8 97168.0
9 97659.0
10 97987.0
11 98224.0
12 98371.0
13 98474.0
14 98546.0
15 98596.0
16 98632.0
17 98657.0
18 98676.0
19 98690.0
20 98702.0
21 98710.0
22 98716.0
23 98721.0
24 98725.0
25 98726.0
26 98726.0
27 98726.0
28 98726.0
29 98726.0
30 98726.0
31 98726.0
32 98726.0
33 98726.0
34 98726.0
35 98726.0
36 98726.0
37 98726.0
38 98726.0
39 98726.0
40 98726.0
41 98726.0
42 98726.0
43 98726.0
44 98726.0
45 98726.0
46 98726.0
47 98726.0
48 98726.0
49 98726.0
50 98726.0
51 98726.0
52 98726.0
53 98726.0
54 98726.0
55 98726.0
56 98726.0
57 98726.0
58 98726.0
59 98726.0
60 98726.0
61 98726.0
62 98726.0
63 98726.0
64 98726.0
65 98726.0
66 98726.0
67 98726.0
68 98726.0
69 98726.0
70 98726.0
71 98726.0
72 98726.0
73 98726.0
74 98726.0
75 98726.0
76 98726.0
77 98726.0
78 98726.0
79 98726.0
80 98726.0
81 98726.0
82 98726.0
83 98726.0
84 98726.0
85 98726.0
86 98726.0
87 98726.0
88 98726.0
89 98726.0
90 98726.0
91 98726.0
92 98726.0
93 98726.0
94 98726.0
95 98726.0
96 98726.0
97 98726.0
98 98726.0
99 98726.0
};
\path [fill=crimson2143940, fill opacity=0.2]
(axis cs:1,9377.0)--
(axis cs:1,9515.2)--
(axis cs:2,14056.2)--
(axis cs:3,17431.1)--
(axis cs:4,20201.1)--
(axis cs:5,22575.1)--
(axis cs:6,24688.0)--
(axis cs:7,26595.9)--
(axis cs:8,28301.1)--
(axis cs:9,29910.5)--
(axis cs:10,31383.8)--
(axis cs:11,32811.5)--
(axis cs:12,34105.3)--
(axis cs:13,35381.1)--
(axis cs:14,36600.2)--
(axis cs:15,37707.4)--
(axis cs:16,38787.4)--
(axis cs:17,39866.9)--
(axis cs:18,40853.7)--
(axis cs:19,41827.2)--
(axis cs:20,42813.8)--
(axis cs:21,43710.9)--
(axis cs:22,44586.0)--
(axis cs:23,45442.9)--
(axis cs:24,46278.8)--
(axis cs:25,47130.1)--
(axis cs:26,47898.9)--
(axis cs:27,48678.7)--
(axis cs:28,49496.0)--
(axis cs:29,50198.2)--
(axis cs:30,50951.0)--
(axis cs:31,51632.3)--
(axis cs:32,52327.2)--
(axis cs:33,53027.4)--
(axis cs:34,53717.1)--
(axis cs:35,54339.5)--
(axis cs:36,55020.2)--
(axis cs:37,55670.4)--
(axis cs:38,56265.0)--
(axis cs:39,56874.3)--
(axis cs:40,57458.0)--
(axis cs:41,58077.3)--
(axis cs:42,58620.2)--
(axis cs:43,59238.2)--
(axis cs:44,59773.4)--
(axis cs:45,60316.3)--
(axis cs:46,60862.1)--
(axis cs:47,61409.2)--
(axis cs:48,61949.4)--
(axis cs:49,62436.7)--
(axis cs:50,62967.6)--
(axis cs:51,63425.2)--
(axis cs:52,63974.1)--
(axis cs:53,64443.0)--
(axis cs:54,64949.6)--
(axis cs:55,65392.1)--
(axis cs:56,65895.4)--
(axis cs:57,66355.8)--
(axis cs:58,66821.6)--
(axis cs:59,67305.5)--
(axis cs:60,67720.4)--
(axis cs:61,68191.2)--
(axis cs:62,68658.1)--
(axis cs:63,69049.4)--
(axis cs:64,69481.3)--
(axis cs:65,69889.2)--
(axis cs:66,70296.1)--
(axis cs:67,70747.3)--
(axis cs:68,71171.0)--
(axis cs:69,71571.7)--
(axis cs:70,71972.0)--
(axis cs:71,72331.6)--
(axis cs:72,72751.3)--
(axis cs:73,73117.6)--
(axis cs:74,73481.6)--
(axis cs:75,73878.6)--
(axis cs:76,74215.6)--
(axis cs:77,74614.4)--
(axis cs:78,74936.4)--
(axis cs:79,75337.1)--
(axis cs:80,75639.7)--
(axis cs:81,75975.0)--
(axis cs:82,76291.6)--
(axis cs:83,76649.0)--
(axis cs:84,76969.1)--
(axis cs:85,77295.2)--
(axis cs:86,77583.3)--
(axis cs:87,77926.1)--
(axis cs:88,78242.2)--
(axis cs:89,78531.9)--
(axis cs:90,78801.3)--
(axis cs:91,79024.1)--
(axis cs:92,79354.1)--
(axis cs:93,79625.4)--
(axis cs:94,79875.1)--
(axis cs:95,80144.7)--
(axis cs:96,80436.7)--
(axis cs:97,80685.4)--
(axis cs:98,80942.5)--
(axis cs:99,81137.5)--
(axis cs:99,80910.4)--
(axis cs:98,80688.1)--
(axis cs:97,80417.9)--
(axis cs:96,80182.4)--
(axis cs:95,79908.3)--
(axis cs:94,79652.8)--
(axis cs:93,79411.7)--
(axis cs:92,79097.4)--
(axis cs:91,78881.2)--
(axis cs:90,78552.7)--
(axis cs:89,78263.6)--
(axis cs:88,77970.9)--
(axis cs:87,77659.0)--
(axis cs:86,77357.5)--
(axis cs:85,77043.8)--
(axis cs:84,76740.3)--
(axis cs:83,76381.9)--
(axis cs:82,76076.8)--
(axis cs:81,75722.4)--
(axis cs:80,75371.9)--
(axis cs:79,75047.7)--
(axis cs:78,74654.0)--
(axis cs:77,74354.6)--
(axis cs:76,73960.2)--
(axis cs:75,73600.9)--
(axis cs:74,73256.6)--
(axis cs:73,72838.8)--
(axis cs:72,72459.7)--
(axis cs:71,72093.6)--
(axis cs:70,71676.2)--
(axis cs:69,71265.7)--
(axis cs:68,70858.0)--
(axis cs:67,70487.4)--
(axis cs:66,70045.0)--
(axis cs:65,69646.3)--
(axis cs:64,69214.9)--
(axis cs:63,68765.9)--
(axis cs:62,68342.6)--
(axis cs:61,67904.7)--
(axis cs:60,67449.9)--
(axis cs:59,67012.2)--
(axis cs:58,66556.5)--
(axis cs:57,66107.9)--
(axis cs:56,65600.8)--
(axis cs:55,65101.5)--
(axis cs:54,64669.9)--
(axis cs:53,64184.3)--
(axis cs:52,63702.4)--
(axis cs:51,63184.1)--
(axis cs:50,62702.5)--
(axis cs:49,62137.4)--
(axis cs:48,61661.8)--
(axis cs:47,61150.8)--
(axis cs:46,60572.8)--
(axis cs:45,60062.8)--
(axis cs:44,59516.5)--
(axis cs:43,58911.9)--
(axis cs:42,58368.4)--
(axis cs:41,57750.9)--
(axis cs:40,57169.9)--
(axis cs:39,56574.8)--
(axis cs:38,55962.8)--
(axis cs:37,55310.8)--
(axis cs:36,54713.6)--
(axis cs:35,54074.6)--
(axis cs:34,53417.4)--
(axis cs:33,52701.2)--
(axis cs:32,52057.5)--
(axis cs:31,51383.8)--
(axis cs:30,50653.2)--
(axis cs:29,49921.8)--
(axis cs:28,49195.5)--
(axis cs:27,48419.1)--
(axis cs:26,47633.7)--
(axis cs:25,46845.0)--
(axis cs:24,46020.9)--
(axis cs:23,45166.1)--
(axis cs:22,44331.0)--
(axis cs:21,43394.0)--
(axis cs:20,42532.0)--
(axis cs:19,41566.4)--
(axis cs:18,40610.3)--
(axis cs:17,39548.7)--
(axis cs:16,38511.9)--
(axis cs:15,37442.1)--
(axis cs:14,36321.4)--
(axis cs:13,35134.0)--
(axis cs:12,33830.0)--
(axis cs:11,32545.7)--
(axis cs:10,31158.9)--
(axis cs:9,29633.6)--
(axis cs:8,28081.7)--
(axis cs:7,26354.5)--
(axis cs:6,24455.7)--
(axis cs:5,22329.1)--
(axis cs:4,19976.7)--
(axis cs:3,17239.7)--
(axis cs:2,13881.6)--
(axis cs:1,9377.0)--
cycle;
\addplot [dashdotted, thick, crimson2143940]
table {%
1 9447.5
2 13959.0
3 17339.0
4 20093.5
5 22465.5
6 24563.5
7 26480.0
8 28198.0
9 29783.0
10 31291.0
11 32678.5
12 33971.0
13 35258.0
14 36464.5
15 37578.5
16 38653.0
17 39719.0
18 40729.5
19 41709.0
20 42659.0
21 43537.5
22 44448.5
23 45339.5
24 46148.5
25 46981.0
26 47783.0
27 48567.5
28 49303.5
29 50081.5
30 50783.5
31 51522.0
32 52197.0
33 52896.0
34 53572.5
35 54209.0
36 54851.5
37 55500.5
38 56101.0
39 56709.0
40 57347.5
41 57944.5
42 58511.5
43 59072.5
44 59633.5
45 60169.5
46 60725.0
47 61275.5
48 61790.0
49 62266.5
50 62840.0
51 63304.0
52 63842.5
53 64317.5
54 64796.0
55 65291.0
56 65762.0
57 66217.0
58 66707.5
59 67178.5
60 67581.0
61 68051.0
62 68498.5
63 68932.5
64 69360.0
65 69745.0
66 70157.0
67 70614.5
68 71030.5
69 71418.0
70 71816.0
71 72215.5
72 72607.0
73 72969.0
74 73358.0
75 73743.0
76 74111.5
77 74459.5
78 74823.0
79 75192.0
80 75518.0
81 75852.0
82 76176.0
83 76520.5
84 76851.0
85 77173.5
86 77466.5
87 77791.0
88 78088.5
89 78381.5
90 78665.5
91 78959.0
92 79238.0
93 79510.5
94 79766.5
95 80023.5
96 80301.5
97 80548.5
98 80795.5
99 81036.0
};
\path [fill=darkgray176, fill opacity=0.2]
(axis cs:1,9392.7)--
(axis cs:1,9512.2)--
(axis cs:2,30634.2)--
(axis cs:3,54829.4)--
(axis cs:4,73451.9)--
(axis cs:5,84413.1)--
(axis cs:6,90397.6)--
(axis cs:7,93691.1)--
(axis cs:8,95549.1)--
(axis cs:9,96665.1)--
(axis cs:10,97358.0)--
(axis cs:11,97811.0)--
(axis cs:12,98103.0)--
(axis cs:13,98298.1)--
(axis cs:14,98429.0)--
(axis cs:15,98515.0)--
(axis cs:16,98576.0)--
(axis cs:17,98619.0)--
(axis cs:18,98650.0)--
(axis cs:19,98674.0)--
(axis cs:20,98689.0)--
(axis cs:21,98703.0)--
(axis cs:22,98712.0)--
(axis cs:23,98718.0)--
(axis cs:24,98722.0)--
(axis cs:25,98725.0)--
(axis cs:26,98726.0)--
(axis cs:27,98726.0)--
(axis cs:28,98726.0)--
(axis cs:29,98726.0)--
(axis cs:30,98726.0)--
(axis cs:31,98726.0)--
(axis cs:32,98726.0)--
(axis cs:33,98726.0)--
(axis cs:34,98726.0)--
(axis cs:35,98726.0)--
(axis cs:36,98726.0)--
(axis cs:37,98726.0)--
(axis cs:38,98726.0)--
(axis cs:39,98726.0)--
(axis cs:40,98726.0)--
(axis cs:41,98726.0)--
(axis cs:42,98726.0)--
(axis cs:43,98726.0)--
(axis cs:44,98726.0)--
(axis cs:45,98726.0)--
(axis cs:46,98726.0)--
(axis cs:47,98726.0)--
(axis cs:48,98726.0)--
(axis cs:49,98726.0)--
(axis cs:50,98726.0)--
(axis cs:51,98726.0)--
(axis cs:52,98726.0)--
(axis cs:53,98726.0)--
(axis cs:54,98726.0)--
(axis cs:55,98726.0)--
(axis cs:56,98726.0)--
(axis cs:57,98726.0)--
(axis cs:58,98726.0)--
(axis cs:59,98726.0)--
(axis cs:60,98726.0)--
(axis cs:61,98726.0)--
(axis cs:62,98726.0)--
(axis cs:63,98726.0)--
(axis cs:64,98726.0)--
(axis cs:65,98726.0)--
(axis cs:66,98726.0)--
(axis cs:67,98726.0)--
(axis cs:68,98726.0)--
(axis cs:69,98726.0)--
(axis cs:70,98726.0)--
(axis cs:71,98726.0)--
(axis cs:72,98726.0)--
(axis cs:73,98726.0)--
(axis cs:74,98726.0)--
(axis cs:75,98726.0)--
(axis cs:76,98726.0)--
(axis cs:77,98726.0)--
(axis cs:78,98726.0)--
(axis cs:79,98726.0)--
(axis cs:80,98726.0)--
(axis cs:81,98726.0)--
(axis cs:82,98726.0)--
(axis cs:83,98726.0)--
(axis cs:84,98726.0)--
(axis cs:85,98726.0)--
(axis cs:86,98726.0)--
(axis cs:87,98726.0)--
(axis cs:88,98726.0)--
(axis cs:89,98726.0)--
(axis cs:90,98726.0)--
(axis cs:91,98726.0)--
(axis cs:92,98726.0)--
(axis cs:93,98726.0)--
(axis cs:94,98726.0)--
(axis cs:95,98726.0)--
(axis cs:96,98726.0)--
(axis cs:97,98726.0)--
(axis cs:98,98726.0)--
(axis cs:99,98726.0)--
(axis cs:99,98726.0)--
(axis cs:98,98726.0)--
(axis cs:97,98726.0)--
(axis cs:96,98726.0)--
(axis cs:95,98726.0)--
(axis cs:94,98726.0)--
(axis cs:93,98726.0)--
(axis cs:92,98726.0)--
(axis cs:91,98726.0)--
(axis cs:90,98726.0)--
(axis cs:89,98726.0)--
(axis cs:88,98726.0)--
(axis cs:87,98726.0)--
(axis cs:86,98726.0)--
(axis cs:85,98726.0)--
(axis cs:84,98726.0)--
(axis cs:83,98726.0)--
(axis cs:82,98726.0)--
(axis cs:81,98726.0)--
(axis cs:80,98726.0)--
(axis cs:79,98726.0)--
(axis cs:78,98726.0)--
(axis cs:77,98726.0)--
(axis cs:76,98726.0)--
(axis cs:75,98726.0)--
(axis cs:74,98726.0)--
(axis cs:73,98726.0)--
(axis cs:72,98726.0)--
(axis cs:71,98726.0)--
(axis cs:70,98726.0)--
(axis cs:69,98726.0)--
(axis cs:68,98726.0)--
(axis cs:67,98726.0)--
(axis cs:66,98726.0)--
(axis cs:65,98726.0)--
(axis cs:64,98726.0)--
(axis cs:63,98726.0)--
(axis cs:62,98726.0)--
(axis cs:61,98726.0)--
(axis cs:60,98726.0)--
(axis cs:59,98726.0)--
(axis cs:58,98726.0)--
(axis cs:57,98726.0)--
(axis cs:56,98726.0)--
(axis cs:55,98726.0)--
(axis cs:54,98726.0)--
(axis cs:53,98726.0)--
(axis cs:52,98726.0)--
(axis cs:51,98726.0)--
(axis cs:50,98726.0)--
(axis cs:49,98726.0)--
(axis cs:48,98726.0)--
(axis cs:47,98726.0)--
(axis cs:46,98726.0)--
(axis cs:45,98726.0)--
(axis cs:44,98726.0)--
(axis cs:43,98726.0)--
(axis cs:42,98726.0)--
(axis cs:41,98726.0)--
(axis cs:40,98726.0)--
(axis cs:39,98726.0)--
(axis cs:38,98726.0)--
(axis cs:37,98726.0)--
(axis cs:36,98726.0)--
(axis cs:35,98726.0)--
(axis cs:34,98726.0)--
(axis cs:33,98726.0)--
(axis cs:32,98726.0)--
(axis cs:31,98726.0)--
(axis cs:30,98726.0)--
(axis cs:29,98726.0)--
(axis cs:28,98726.0)--
(axis cs:27,98725.0)--
(axis cs:26,98724.0)--
(axis cs:25,98721.0)--
(axis cs:24,98718.0)--
(axis cs:23,98712.0)--
(axis cs:22,98704.0)--
(axis cs:21,98694.0)--
(axis cs:20,98679.0)--
(axis cs:19,98662.0)--
(axis cs:18,98637.0)--
(axis cs:17,98606.0)--
(axis cs:16,98561.0)--
(axis cs:15,98496.0)--
(axis cs:14,98405.0)--
(axis cs:13,98268.0)--
(axis cs:12,98067.9)--
(axis cs:11,97766.0)--
(axis cs:10,97311.0)--
(axis cs:9,96610.6)--
(axis cs:8,95487.9)--
(axis cs:7,93601.8)--
(axis cs:6,90270.9)--
(axis cs:5,84223.8)--
(axis cs:4,73170.6)--
(axis cs:3,54447.2)--
(axis cs:2,30311.8)--
(axis cs:1,9392.7)--
cycle;
% \addplot [thick, darkgray176]
% table {%
% 1 9450.0
% 2 30484.5
% 3 54636.5
% 4 73316.5
% 5 84308.5
% 6 90343.5
% 7 93646.5
% 8 95520.5
% 9 96640.5
% 10 97332.0
% 11 97790.0
% 12 98083.0
% 13 98284.0
% 14 98418.0
% 15 98506.5
% 16 98569.0
% 17 98613.0
% 18 98644.0
% 19 98668.0
% 20 98685.0
% 21 98698.5
% 22 98708.0
% 23 98715.0
% 24 98720.0
% 25 98723.0
% 26 98725.0
% 27 98726.0
% 28 98726.0
% 29 98726.0
% 30 98726.0
% 31 98726.0
% 32 98726.0
% 33 98726.0
% 34 98726.0
% 35 98726.0
% 36 98726.0
% 37 98726.0
% 38 98726.0
% 39 98726.0
% 40 98726.0
% 41 98726.0
% 42 98726.0
% 43 98726.0
% 44 98726.0
% 45 98726.0
% 46 98726.0
% 47 98726.0
% 48 98726.0
% 49 98726.0
% 50 98726.0
% 51 98726.0
% 52 98726.0
% 53 98726.0
% 54 98726.0
% 55 98726.0
% 56 98726.0
% 57 98726.0
% 58 98726.0
% 59 98726.0
% 60 98726.0
% 61 98726.0
% 62 98726.0
% 63 98726.0
% 64 98726.0
% 65 98726.0
% 66 98726.0
% 67 98726.0
% 68 98726.0
% 69 98726.0
% 70 98726.0
% 71 98726.0
% 72 98726.0
% 73 98726.0
% 74 98726.0
% 75 98726.0
% 76 98726.0
% 77 98726.0
% 78 98726.0
% 79 98726.0
% 80 98726.0
% 81 98726.0
% 82 98726.0
% 83 98726.0
% 84 98726.0
% 85 98726.0
% 86 98726.0
% 87 98726.0
% 88 98726.0
% 89 98726.0
% 90 98726.0
% 91 98726.0
% 92 98726.0
% 93 98726.0
% 94 98726.0
% 95 98726.0
% 96 98726.0
% 97 98726.0
% 98 98726.0
% 99 98726.0
% };


==> figures/epsilon/amazon_fashion.tex <==
\nextgroupplot [
    title=Amazon Fashion,
    xmin=1, xmax=30,
    ymin=1421, ymax=1464,
    ylabel={Distinct Count},
    legend style = {
        column sep = 10pt,
        legend columns = 2, 
        legend to name = epsilongrouplegend,
        draw=none
    }
]
\addplot [dashed, steelblue31119180]
table {%
1 1450
2 1450
3 1450
4 1450
5 1450
6 1450
7 1450
8 1450
9 1450
10 1450
11 1450
12 1450
13 1450
14 1450
15 1450
16 1450
17 1450
18 1450
19 1450
20 1450
21 1450
22 1450
23 1450
24 1450
25 1450
26 1450
27 1450
28 1450
29 1450
};
\path [fill=forestgreen4416044, fill opacity=0.2]
(axis cs:1,1217.697613887527)--
(axis cs:1,1381.2359948763078)--
(axis cs:2,1432.4034175066172)--
(axis cs:3,1436.932071181043)--
(axis cs:4,1441.1197313277908)--
(axis cs:5,1440.838737101001)--
(axis cs:6,1443.9273888877133)--
(axis cs:7,1445.205213283387)--
(axis cs:8,1443.0022501863227)--
(axis cs:9,1446.8403565689373)--
(axis cs:10,1446.6440433781236)--
(axis cs:11,1446.0157521146493)--
(axis cs:12,1446.0898454835576)--
(axis cs:13,1448.8374032582328)--
(axis cs:14,1449.0816982949952)--
(axis cs:15,1446.9661912972444)--
(axis cs:16,1447.1285387438047)--
(axis cs:17,1446.6593952332914)--
(axis cs:18,1448.503280585947)--
(axis cs:19,1447.7991036037088)--
(axis cs:20,1449.0183022539168)--
(axis cs:21,1449.2172413667108)--
(axis cs:22,1448.8035209873256)--
(axis cs:23,1449.1703219222086)--
(axis cs:24,1449.042458723308)--
(axis cs:25,1450.5067034915521)--
(axis cs:26,1448.5364301506254)--
(axis cs:27,1450.1554753529388)--
(axis cs:28,1449.6447972985088)--
(axis cs:29,1449.5852773907795)--
(axis cs:29,1436.7641399836666)--
(axis cs:28,1437.9067078568926)--
(axis cs:27,1433.8908644501428)--
(axis cs:26,1433.1230925817351)--
(axis cs:25,1436.593767121295)--
(axis cs:24,1433.2858116252778)--
(axis cs:23,1433.3812279538997)--
(axis cs:22,1432.2122024006644)--
(axis cs:21,1430.56785526584)--
(axis cs:20,1430.361442436269)--
(axis cs:19,1427.060994774941)--
(axis cs:18,1427.6891634661035)--
(axis cs:17,1427.2511214303354)--
(axis cs:16,1425.2182766110382)--
(axis cs:15,1424.4758787534213)--
(axis cs:14,1426.4989664501638)--
(axis cs:13,1417.1772503056116)--
(axis cs:12,1420.0368571867014)--
(axis cs:11,1418.1472183414303)--
(axis cs:10,1411.4507328586128)--
(axis cs:9,1407.3618986757756)--
(axis cs:8,1405.997726030041)--
(axis cs:7,1405.633304319763)--
(axis cs:6,1394.0011855333112)--
(axis cs:5,1376.9149662235718)--
(axis cs:4,1367.5053767453942)--
(axis cs:3,1342.37436612341)--
(axis cs:2,1312.1830511309129)--
(axis cs:1,1217.697613887527)--
cycle;
\addplot [densely dotted, thick, forestgreen4416044]
table {%
1 1311.9101057697037
2 1383.2681089068783
3 1398.6856122160398
4 1416.9196982301874
5 1420.3562227434818
6 1426.50804641889
7 1429.65569047893
8 1428.5859332059233
9 1430.7568016770083
10 1435.3758614409544
11 1436.3466063367491
12 1434.8037464619465
13 1439.4289644418639
14 1439.043706256733
15 1439.007468330266
16 1440.505581584497
17 1439.5318659837576
18 1440.4874384203176
19 1439.597386699897
20 1441.8557664573489
21 1442.5762563506387
22 1442.0007930997735
23 1441.8299173276991
24 1442.9125259241891
25 1443.8495663085732
26 1443.7628086975024
27 1444.4866109498648
28 1444.4389191516798
29 1444.1853961841898
};
\path [fill=darkorange25512714, fill opacity=0.2]
(axis cs:1,1127.4698039307928)--
(axis cs:1,1369.9089090394684)--
(axis cs:2,1409.2397734237102)--
(axis cs:3,1427.765868580942)--
(axis cs:4,1441.8797748505558)--
(axis cs:5,1438.5464163072568)--
(axis cs:6,1441.2709024890287)--
(axis cs:7,1442.8416425097992)--
(axis cs:8,1446.1173513567578)--
(axis cs:9,1445.2970974828795)--
(axis cs:10,1443.9432317615422)--
(axis cs:11,1448.6610470203568)--
(axis cs:12,1448.9606937501685)--
(axis cs:13,1446.6872241023643)--
(axis cs:14,1449.9931169776942)--
(axis cs:15,1447.8633147966873)--
(axis cs:16,1447.8871438751041)--
(axis cs:17,1447.925559674634)--
(axis cs:18,1449.3827162671018)--
(axis cs:19,1447.886606452137)--
(axis cs:20,1451.3638017420883)--
(axis cs:21,1448.3195523671452)--
(axis cs:22,1449.6230336552849)--
(axis cs:23,1447.9741855838304)--
(axis cs:24,1449.7132663078446)--
(axis cs:25,1448.3934789433995)--
(axis cs:26,1448.2168415160343)--
(axis cs:27,1448.779576111942)--
(axis cs:28,1449.6236757454549)--
(axis cs:29,1449.8067483310208)--
(axis cs:29,1436.4856121280827)--
(axis cs:28,1436.9481034401426)--
(axis cs:27,1430.3417440517883)--
(axis cs:26,1433.9915420160673)--
(axis cs:25,1433.9204263042247)--
(axis cs:24,1430.0746317183446)--
(axis cs:23,1432.2065755081628)--
(axis cs:22,1431.431406541105)--
(axis cs:21,1430.619558787817)--
(axis cs:20,1430.4786977167323)--
(axis cs:19,1428.810166450662)--
(axis cs:18,1425.5302407513832)--
(axis cs:17,1424.7836196671856)--
(axis cs:16,1422.8584914028181)--
(axis cs:15,1426.0462446142235)--
(axis cs:14,1412.0789298475327)--
(axis cs:13,1416.4721527467698)--
(axis cs:12,1406.94360281784)--
(axis cs:11,1403.1506493585557)--
(axis cs:10,1406.0416919046102)--
(axis cs:9,1400.7918936676701)--
(axis cs:8,1384.9288104704272)--
(axis cs:7,1380.3457906480578)--
(axis cs:6,1386.860808440827)--
(axis cs:5,1344.1435628174236)--
(axis cs:4,1339.0026969825662)--
(axis cs:3,1308.2224841357424)--
(axis cs:2,1260.211665592377)--
(axis cs:1,1127.4698039307928)--
cycle;
\addplot [densely dotted, thick, darkorange25512714]
table {%
1 1267.8146549460903
2 1351.2288567749042
3 1385.9159021804453
4 1396.5868775687886
5 1410.5958688284018
6 1421.1926849679526
7 1425.6514120245397
8 1429.5403064174698
9 1430.7984427650704
10 1431.2771424882064
11 1431.4201684853288
12 1435.108291448588
13 1438.6753203941494
14 1435.1159409313293
15 1437.9776256896685
16 1440.8650878361464
17 1439.5958261935189
18 1440.998876148286
19 1439.0202841965056
20 1441.3756268069383
21 1442.0262750239901
22 1442.6303888968084
23 1443.3690665985882
24 1442.5939985641592
25 1442.8237842579
26 1443.9158784901083
27 1443.4957648888017
28 1445.0563902211888
29 1445.5687781977226
};
\path [fill=crimson2143940, fill opacity=0.2]
(axis cs:1,598.3146715235763)--
(axis cs:1,1124.3261063054172)--
(axis cs:2,1247.72044702286)--
(axis cs:3,1357.467625517095)--
(axis cs:4,1374.5466974646324)--
(axis cs:5,1369.1686361924283)--
(axis cs:6,1369.3379849581504)--
(axis cs:7,1401.6488504035303)--
(axis cs:8,1405.7302055769962)--
(axis cs:9,1395.5936478393369)--
(axis cs:10,1404.1482242266177)--
(axis cs:11,1413.1189269498068)--
(axis cs:12,1407.7128634646042)--
(axis cs:13,1417.9591540809251)--
(axis cs:14,1410.1386666273158)--
(axis cs:15,1410.7693579692482)--
(axis cs:16,1417.0366195598283)--
(axis cs:17,1418.677152835403)--
(axis cs:18,1422.165746466908)--
(axis cs:19,1419.1510523552793)--
(axis cs:20,1416.2501194408635)--
(axis cs:21,1423.183340389413)--
(axis cs:22,1418.421417181901)--
(axis cs:23,1422.5438595144656)--
(axis cs:24,1420.6383976309346)--
(axis cs:25,1423.157625080997)--
(axis cs:26,1423.6076728652165)--
(axis cs:27,1421.096438340958)--
(axis cs:28,1423.220743984437)--
(axis cs:29,1427.6276227613791)--
(axis cs:29,1353.4098802645)--
(axis cs:28,1358.8232575258974)--
(axis cs:27,1360.8138770174735)--
(axis cs:26,1362.3863783334405)--
(axis cs:25,1360.3503264515061)--
(axis cs:24,1344.148021183609)--
(axis cs:23,1334.298887912937)--
(axis cs:22,1341.9638133028407)--
(axis cs:21,1349.3322979395423)--
(axis cs:20,1351.6913441815454)--
(axis cs:19,1315.5309268491515)--
(axis cs:18,1331.4089601533076)--
(axis cs:17,1319.2655141749283)--
(axis cs:16,1324.230628031098)--
(axis cs:15,1311.8634083086304)--
(axis cs:14,1298.5862364315788)--
(axis cs:13,1305.0398274859083)--
(axis cs:12,1297.960177084517)--
(axis cs:11,1252.1343278409206)--
(axis cs:10,1270.4615672618409)--
(axis cs:9,1269.6118266449637)--
(axis cs:8,1213.7765649914827)--
(axis cs:7,1225.3968701336019)--
(axis cs:6,1205.1089326080032)--
(axis cs:5,1127.6231993626643)--
(axis cs:4,1098.255326253167)--
(axis cs:3,1038.356511512096)--
(axis cs:2,897.9491575479967)--
(axis cs:1,598.3146715235763)--
cycle;
\addplot [dashdotted, thick, crimson2143940]
table {%
1 858.622451668276
2 1107.356579210428
3 1201.8065145415667
4 1247.0519867042917
5 1278.2432442789623
6 1299.3215927643419
7 1314.4518055078352
8 1324.1603110966937
9 1324.978583161268
10 1345.5087547394837
11 1352.9692070883184
12 1360.7050705415018
13 1367.2965419922666
14 1354.0946443468613
15 1371.1162870482551
16 1380.6142189836924
17 1384.3413358244457
18 1383.5328184619898
19 1382.5574971867422
20 1388.891738564638
21 1398.9209244325343
22 1393.2723183974854
23 1392.610676524492
24 1394.7750605232277
25 1403.9331013612364
26 1404.6160638570977
27 1400.2121545428322
28 1397.9453696712908
29 1405.1016112863265
};

\path [fill=steelblue31119180, fill opacity=0.2]
(axis cs:1,972.8)--
(axis cs:1,1377.3)--
(axis cs:2,1428.0)--
(axis cs:3,1440.0)--
(axis cs:4,1433.1)--
(axis cs:5,1445.2)--
(axis cs:6,1450.0)--
(axis cs:7,1437.0)--
(axis cs:8,1451.0)--
(axis cs:9,1443.7)--
(axis cs:10,1451.0)--
(axis cs:11,1450.0)--
(axis cs:12,1451.0)--
(axis cs:13,1451.0)--
(axis cs:14,1451.0)--
(axis cs:15,1451.0)--
(axis cs:16,1451.0)--
(axis cs:17,1451.0)--
(axis cs:18,1450.1)--
(axis cs:19,1450.0)--
(axis cs:20,1451.0)--
(axis cs:21,1451.0)--
(axis cs:22,1451.0)--
(axis cs:23,1451.0)--
(axis cs:24,1451.0)--
(axis cs:25,1451.0)--
(axis cs:26,1451.0)--
(axis cs:27,1451.0)--
(axis cs:28,1451.0)--
(axis cs:29,1451.0)--
(axis cs:29,1426.9)--
(axis cs:28,1430.9)--
(axis cs:27,1432.9)--
(axis cs:26,1430.0)--
(axis cs:25,1428.0)--
(axis cs:24,1427.0)--
(axis cs:23,1426.0)--
(axis cs:22,1385.8)--
(axis cs:21,1385.0)--
(axis cs:20,1388.9)--
(axis cs:19,1386.8)--
(axis cs:18,1387.9)--
(axis cs:17,1391.8)--
(axis cs:16,1388.0)--
(axis cs:15,1388.0)--
(axis cs:14,1388.7)--
(axis cs:13,1386.0)--
(axis cs:12,1392.9)--
(axis cs:11,1359.7)--
(axis cs:10,1356.9)--
(axis cs:9,1353.0)--
(axis cs:8,1353.0)--
(axis cs:7,1323.0)--
(axis cs:6,1321.8)--
(axis cs:5,1294.0)--
(axis cs:4,1265.5)--
(axis cs:3,1220.0)--
(axis cs:2,1142.6)--
(axis cs:1,972.8)--
cycle;
\addplot [dashdotted, thick, steelblue31119180]
table {%
1 1128.0
2 1264.5
3 1299.5
4 1333.5
5 1372.0
6 1380.5
7 1374.5
8 1401.0
9 1385.5
10 1411.0
11 1403.5
12 1428.0
13 1422.0
14 1422.0
15 1419.0
16 1426.0
17 1424.5
18 1430.0
19 1421.0
20 1423.0
21 1424.0
22 1422.5
23 1449.0
24 1449.0
25 1450.0
26 1448.5
27 1450.0
28 1450.0
29 1450.0
};



\addlegendentry{true value}
\addlegendentry{matching algorithm}
\addlegendentry{greedy algorithm}
\addlegendentry{sampling algorithm}
\addlegendentry{shifted inverse algorithm}

==> figures/epsilon/amazon_industrial.tex <==
\nextgroupplot [
    title=Amazon Industrial,,
    xmin=1, xmax=30,
    ymin=35931.7, ymax=37031.65
]
\addplot [dashed, steelblue31119180]
table {%
1 36665
2 36665
3 36665
4 36665
5 36665
6 36665
7 36665
8 36665
9 36665
10 36665
11 36665
12 36665
13 36665
14 36665
15 36665
16 36665
17 36665
18 36665
19 36665
20 36665
21 36665
22 36665
23 36665
24 36665
25 36665
26 36665
27 36665
28 36665
29 36665
};
\path [fill=forestgreen4416044, fill opacity=0.2]
(axis cs:1,35786.69734587706)--
(axis cs:1,36316.14201337107)--
(axis cs:2,36390.171313396626)--
(axis cs:3,36482.77429032042)--
(axis cs:4,36500.660836280695)--
(axis cs:5,36512.93613635334)--
(axis cs:6,36531.12996752278)--
(axis cs:7,36568.47194853353)--
(axis cs:8,36562.69497834038)--
(axis cs:9,36545.02821335793)--
(axis cs:10,36560.807393641)--
(axis cs:11,36564.472068328396)--
(axis cs:12,36570.62240994522)--
(axis cs:13,36574.84341686273)--
(axis cs:14,36580.838412873156)--
(axis cs:15,36573.94548373256)--
(axis cs:16,36575.62595396624)--
(axis cs:17,36581.467509622555)--
(axis cs:18,36576.114281040645)--
(axis cs:19,36580.857630271974)--
(axis cs:20,36587.50709299556)--
(axis cs:21,36581.66054800869)--
(axis cs:22,36581.33728501855)--
(axis cs:23,36586.047805526614)--
(axis cs:24,36584.378058798866)--
(axis cs:25,36583.53042860866)--
(axis cs:26,36583.211095984414)--
(axis cs:27,36586.77752191941)--
(axis cs:28,36585.28817675553)--
(axis cs:29,36586.334557980874)--
(axis cs:29,36518.81271967996)--
(axis cs:28,36527.74925785466)--
(axis cs:27,36494.65999368357)--
(axis cs:26,36511.723012117895)--
(axis cs:25,36502.530371861336)--
(axis cs:24,36507.420937930285)--
(axis cs:23,36495.68050937723)--
(axis cs:22,36495.28555443711)--
(axis cs:21,36468.99828758835)--
(axis cs:20,36503.14359510622)--
(axis cs:19,36485.78358067948)--
(axis cs:18,36459.349389324496)--
(axis cs:17,36456.54964021807)--
(axis cs:16,36464.342391390805)--
(axis cs:15,36446.970875411644)--
(axis cs:14,36438.87539671419)--
(axis cs:13,36418.24894343417)--
(axis cs:12,36411.63176445215)--
(axis cs:11,36408.24456449064)--
(axis cs:10,36385.68567977879)--
(axis cs:9,36385.71931797666)--
(axis cs:8,36356.809742230565)--
(axis cs:7,36326.20626878007)--
(axis cs:6,36305.19972233886)--
(axis cs:5,36314.24454942238)--
(axis cs:4,36252.51103209409)--
(axis cs:3,36216.822757544345)--
(axis cs:2,36083.89572335366)--
(axis cs:1,35786.69734587706)--
cycle;
\addplot [densely dotted, thick, forestgreen4416044]
table {%
1 36098.69663520448
2 36269.25160793646
3 36347.90281978053
4 36368.66082701442
5 36412.33352649156
6 36420.636870178554
7 36434.964637121026
8 36460.64906831189
9 36478.33519151383
10 36475.23305573855
11 36508.421021932416
12 36514.44369886951
13 36515.84655676744
14 36523.16199919257
15 36514.368671992605
16 36544.75011637938
17 36548.57206529188
18 36538.56740809957
19 36550.50527722184
20 36558.954324380255
21 36544.002620732455
22 36552.391926857235
23 36562.200514635304
24 36553.75527513065
25 36558.1446310375
26 36564.060294763105
27 36561.816607854475
28 36570.41770225478
29 36566.96544795894
};
\path [fill=darkorange25512714, fill opacity=0.2]
(axis cs:1,35745.875365181266)--
(axis cs:1,36324.85818378764)--
(axis cs:2,36396.46370570858)--
(axis cs:3,36457.98625125203)--
(axis cs:4,36485.705759259516)--
(axis cs:5,36498.124573863905)--
(axis cs:6,36540.682692651586)--
(axis cs:7,36529.76468811314)--
(axis cs:8,36544.88087202535)--
(axis cs:9,36557.19280831943)--
(axis cs:10,36558.20182534925)--
(axis cs:11,36565.518775364086)--
(axis cs:12,36565.22457631038)--
(axis cs:13,36565.101085944014)--
(axis cs:14,36569.793439846886)--
(axis cs:15,36575.65567177794)--
(axis cs:16,36574.95110159735)--
(axis cs:17,36577.747281147946)--
(axis cs:18,36578.95706890639)--
(axis cs:19,36574.985797546586)--
(axis cs:20,36576.78669637204)--
(axis cs:21,36581.08481492417)--
(axis cs:22,36581.39164794443)--
(axis cs:23,36581.607847864965)--
(axis cs:24,36582.72557201446)--
(axis cs:25,36580.15014370763)--
(axis cs:26,36585.15983541677)--
(axis cs:27,36582.57759323054)--
(axis cs:28,36579.97818653861)--
(axis cs:29,36583.340768702146)--
(axis cs:29,36523.85426020103)--
(axis cs:28,36509.2011867445)--
(axis cs:27,36508.96437971436)--
(axis cs:26,36517.186170945286)--
(axis cs:25,36509.992437243796)--
(axis cs:24,36498.28255837841)--
(axis cs:23,36502.44877913289)--
(axis cs:22,36480.64301996155)--
(axis cs:21,36480.49429257588)--
(axis cs:20,36465.435905679755)--
(axis cs:19,36459.382164274655)--
(axis cs:18,36486.89539853341)--
(axis cs:17,36475.36990601222)--
(axis cs:16,36458.85017360816)--
(axis cs:15,36437.87174651485)--
(axis cs:14,36452.16767549263)--
(axis cs:13,36412.54667574015)--
(axis cs:12,36403.25182084639)--
(axis cs:11,36404.104547182564)--
(axis cs:10,36360.528757007385)--
(axis cs:9,36376.36563792391)--
(axis cs:8,36358.6870517469)--
(axis cs:7,36342.07195736957)--
(axis cs:6,36300.94046505994)--
(axis cs:5,36285.221082448734)--
(axis cs:4,36257.32337222797)--
(axis cs:3,36143.57465937899)--
(axis cs:2,36074.6797050248)--
(axis cs:1,35745.875365181266)--
cycle;
\addplot [densely dotted, thick, darkorange25512714]
table {%
1 36079.023872326215
2 36261.66524960086
3 36313.96931712044
4 36372.76286438311
5 36385.9182884332
6 36414.32012806897
7 36436.2961221797
8 36464.63730072584
9 36463.66802627139
10 36481.27183033392
11 36487.52769530346
12 36501.127381303464
13 36522.136644496175
14 36526.2651916889
15 36524.5184385178
16 36539.283507650085
17 36550.46943190082
18 36547.643148900024
19 36542.303938718345
20 36549.37240969713
21 36549.04888100041
22 36549.64446342416
23 36557.20696170526
24 36559.95108459141
25 36558.679369562786
26 36565.68069007152
27 36562.91983488171
28 36558.006578226355
29 36560.78846501195
};
\path [fill=crimson2143940, fill opacity=0.2]
(axis cs:1,23033.334984082383)--
(axis cs:1,25003.510129892184)--
(axis cs:2,24978.316988574257)--
(axis cs:3,25017.661638597114)--
(axis cs:4,25044.431600420718)--
(axis cs:5,25043.135618244425)--
(axis cs:6,25055.864902370653)--
(axis cs:7,25103.30314237621)--
(axis cs:8,25086.127874853755)--
(axis cs:9,25068.493265437337)--
(axis cs:10,25116.056387290828)--
(axis cs:11,25121.285465451132)--
(axis cs:12,25087.251773102307)--
(axis cs:13,25122.879154948114)--
(axis cs:14,25089.060715432257)--
(axis cs:15,25091.646306523133)--
(axis cs:16,25081.414767171125)--
(axis cs:17,25105.371441680792)--
(axis cs:18,25117.27025649805)--
(axis cs:19,25104.862747568663)--
(axis cs:20,25099.697423599504)--
(axis cs:21,25088.347841033123)--
(axis cs:22,25101.186355886464)--
(axis cs:23,25082.474143761665)--
(axis cs:24,25104.28977087416)--
(axis cs:25,25093.57509490375)--
(axis cs:26,25112.20794665283)--
(axis cs:27,25087.96630663446)--
(axis cs:28,25093.474996520927)--
(axis cs:29,25086.584973196925)--
(axis cs:29,24911.999647746936)--
(axis cs:28,24935.44937111891)--
(axis cs:27,24916.40091492501)--
(axis cs:26,24942.897381393926)--
(axis cs:25,24920.42902140647)--
(axis cs:24,24911.721856857483)--
(axis cs:23,24915.855136594615)--
(axis cs:22,24875.789091057326)--
(axis cs:21,24906.639754373275)--
(axis cs:20,24918.664159248005)--
(axis cs:19,24902.80373630342)--
(axis cs:18,24905.678920897928)--
(axis cs:17,24901.30133608685)--
(axis cs:16,24911.941356914296)--
(axis cs:15,24871.38288853461)--
(axis cs:14,24836.312221875392)--
(axis cs:13,24847.81905095252)--
(axis cs:12,24849.16307026185)--
(axis cs:11,24842.644748932245)--
(axis cs:10,24844.285140257445)--
(axis cs:9,24804.963528730008)--
(axis cs:8,24822.897168541625)--
(axis cs:7,24771.112771947406)--
(axis cs:6,24714.089965744824)--
(axis cs:5,24675.92247993275)--
(axis cs:4,24572.124016034166)--
(axis cs:3,24382.498082504975)--
(axis cs:2,23860.07393580274)--
(axis cs:1,23033.334984082383)--
cycle;
\addplot [dashdotted, thick, crimson2143940]
table {%
1 24150.56553648814
2 24680.820846087743
3 24767.895085370685
4 24868.841280095847
5 24924.63460820219
6 24942.612613320372
7 24978.522593655878
8 24970.51623637731
9 24987.530913036957
10 24982.270871225406
11 24992.4331251401
12 25001.97573782681
13 25006.386519171378
14 25001.196003691584
15 25004.94841231578
16 24999.365273969874
17 25021.273517243135
18 25022.781853327124
19 25010.692378615364
20 25028.432021088425
21 25012.106295952577
22 24992.39929433689
23 24995.987977460416
24 25027.771935960714
25 25003.780097256982
26 25018.854240602923
27 25021.761850780844
28 25029.39442124075
29 25009.775354482394
};

\path [fill=steelblue31119180, fill opacity=0.2]
(axis cs:1,35156.0)--
(axis cs:1,36244.2)--
(axis cs:2,36459.9)--
(axis cs:3,36554.1)--
(axis cs:4,36605.4)--
(axis cs:5,36641.5)--
(axis cs:6,36700.7)--
(axis cs:7,36677.1)--
(axis cs:8,36711.4)--
(axis cs:9,36700.1)--
(axis cs:10,36684.3)--
(axis cs:11,36703.2)--
(axis cs:12,36715.1)--
(axis cs:13,36713.0)--
(axis cs:14,36709.2)--
(axis cs:15,36701.1)--
(axis cs:16,36690.4)--
(axis cs:17,36706.2)--
(axis cs:18,36701.0)--
(axis cs:19,36701.6)--
(axis cs:20,36708.2)--
(axis cs:21,36703.6)--
(axis cs:22,36706.1)--
(axis cs:23,36719.0)--
(axis cs:24,36714.1)--
(axis cs:25,36717.0)--
(axis cs:26,36714.1)--
(axis cs:27,36715.1)--
(axis cs:28,36720.1)--
(axis cs:29,36715.2)--
(axis cs:29,36579.8)--
(axis cs:28,36581.9)--
(axis cs:27,36605.9)--
(axis cs:26,36587.0)--
(axis cs:25,36602.4)--
(axis cs:24,36604.2)--
(axis cs:23,36600.6)--
(axis cs:22,36365.2)--
(axis cs:21,36362.0)--
(axis cs:20,36378.7)--
(axis cs:19,36341.5)--
(axis cs:18,36397.6)--
(axis cs:17,36363.2)--
(axis cs:16,36395.0)--
(axis cs:15,36352.9)--
(axis cs:14,36350.8)--
(axis cs:13,36395.7)--
(axis cs:12,36392.4)--
(axis cs:11,36224.0)--
(axis cs:10,36224.0)--
(axis cs:9,36224.0)--
(axis cs:8,36224.0)--
(axis cs:7,36140.0)--
(axis cs:6,36140.0)--
(axis cs:5,36060.8)--
(axis cs:4,36023.5)--
(axis cs:3,35892.0)--
(axis cs:2,35680.8)--
(axis cs:1,35156.0)--
cycle;
\addplot [dashdotted, thick, steelblue31119180]
table {%
1 35652.5
2 35973.5
3 36102.5
4 36140.0
5 36224.0
6 36369.5
7 36357.0
8 36479.0
9 36503.0
10 36488.0
11 36440.5
12 36555.5
13 36578.5
14 36580.0
15 36580.0
16 36528.0
17 36532.0
18 36550.0
19 36556.5
20 36570.0
21 36579.0
22 36548.5
23 36682.5
24 36686.0
25 36676.5
26 36676.0
27 36681.0
28 36677.5
29 36675.5
};



==> figures/epsilon/askreddit.tex <==
\nextgroupplot [
    title=Reddit,
    xmin=1, xmax=30,
    ymin=102579, ymax=102963,
    ylabel={Distinct Count},
]

\addplot [dashed, steelblue31119180]
table {%
1 102835
2 102835
3 102835
4 102835
5 102835
6 102835
7 102835
8 102835
9 102835
10 102835
11 102835
12 102835
13 102835
14 102835
15 102835
16 102835
17 102835
18 102835
19 102835
20 102835
21 102835
22 102835
23 102835
24 102835
25 102835
26 102835
27 102835
28 102835
29 102835
};
\path [fill=forestgreen4416044, fill opacity=0.2]
(axis cs:1,102206.0977971804)--
(axis cs:1,102610.3864947537)--
(axis cs:2,102712.65270554066)--
(axis cs:3,102728.8873262764)--
(axis cs:4,102735.35298981896)--
(axis cs:5,102765.85382810776)--
(axis cs:6,102764.60691087223)--
(axis cs:7,102778.46120093625)--
(axis cs:8,102791.26738643022)--
(axis cs:9,102788.91322278582)--
(axis cs:10,102792.09732907849)--
(axis cs:11,102799.2547694256)--
(axis cs:12,102787.53078688585)--
(axis cs:13,102790.21298539493)--
(axis cs:14,102797.17175858827)--
(axis cs:15,102793.2978951962)--
(axis cs:16,102795.50062934695)--
(axis cs:17,102800.03167844312)--
(axis cs:18,102808.91197710251)--
(axis cs:19,102807.19676707861)--
(axis cs:20,102803.6583837275)--
(axis cs:21,102800.10790072197)--
(axis cs:22,102805.83364651755)--
(axis cs:23,102801.28878773138)--
(axis cs:24,102801.35640383762)--
(axis cs:25,102811.45032643015)--
(axis cs:26,102813.46745076026)--
(axis cs:27,102810.76062806924)--
(axis cs:28,102811.40072778672)--
(axis cs:29,102809.45956039336)--
(axis cs:29,102756.35411782829)--
(axis cs:28,102759.80934250029)--
(axis cs:27,102767.852193838)--
(axis cs:26,102763.7235285407)--
(axis cs:25,102750.34346132011)--
(axis cs:24,102745.23828672677)--
(axis cs:23,102752.65441859719)--
(axis cs:22,102748.42338520108)--
(axis cs:21,102744.62707878742)--
(axis cs:20,102733.27810371012)--
(axis cs:19,102734.7685167111)--
(axis cs:18,102731.59005037724)--
(axis cs:17,102722.84501604452)--
(axis cs:16,102728.99274773024)--
(axis cs:15,102724.51770819693)--
(axis cs:14,102724.42157211245)--
(axis cs:13,102702.8910835059)--
(axis cs:12,102711.91196117736)--
(axis cs:11,102687.19257151242)--
(axis cs:10,102699.74528668549)--
(axis cs:9,102674.66148876843)--
(axis cs:8,102663.27409683603)--
(axis cs:7,102643.44465808177)--
(axis cs:6,102621.74321459277)--
(axis cs:5,102622.26162841415)--
(axis cs:4,102591.48863486762)--
(axis cs:3,102514.83961813447)--
(axis cs:2,102471.12465775642)--
(axis cs:1,102206.0977971804)--
cycle;
\addplot [densely dotted, thick, forestgreen4416044]
table {%
1 102463.53277235595
2 102611.08245053276
3 102661.21856307883
4 102680.20565631674
5 102694.90383898473
6 102706.46379359654
7 102733.27875771327
8 102739.46037044076
9 102738.5556132542
10 102759.2273343887
11 102746.67018124138
12 102765.99546424473
13 102758.53059828834
14 102763.98965827908
15 102765.98978677465
16 102769.52466285702
17 102773.93861400093
18 102771.44256942556
19 102780.95277149134
20 102774.67006945255
21 102777.3309485618
22 102783.45377763594
23 102781.10358895075
24 102780.75618060789
25 102789.83220891102
26 102792.19878632828
27 102791.64250452715
28 102790.83354144396
29 102788.71396463926
};
\path [fill=darkorange25512714, fill opacity=0.2]
(axis cs:1,102263.46617295791)--
(axis cs:1,102636.5447172141)--
(axis cs:2,102696.85873147342)--
(axis cs:3,102727.6591735613)--
(axis cs:4,102753.99854179824)--
(axis cs:5,102775.31772147019)--
(axis cs:6,102771.02227861155)--
(axis cs:7,102779.17170303034)--
(axis cs:8,102781.17660031747)--
(axis cs:9,102781.43274661784)--
(axis cs:10,102793.35896651879)--
(axis cs:11,102793.28161373727)--
(axis cs:12,102790.77226826394)--
(axis cs:13,102789.70267553219)--
(axis cs:14,102801.51638869458)--
(axis cs:15,102798.77035117676)--
(axis cs:16,102793.1723411888)--
(axis cs:17,102802.14946138648)--
(axis cs:18,102799.55566675532)--
(axis cs:19,102801.95513282665)--
(axis cs:20,102803.59285916574)--
(axis cs:21,102806.92292717707)--
(axis cs:22,102809.25012597487)--
(axis cs:23,102810.31714809024)--
(axis cs:24,102805.48973710132)--
(axis cs:25,102804.75338333378)--
(axis cs:26,102804.01520543698)--
(axis cs:27,102808.9488352983)--
(axis cs:28,102809.83352317213)--
(axis cs:29,102807.65487921632)--
(axis cs:29,102757.98528402978)--
(axis cs:28,102752.23046021114)--
(axis cs:27,102759.16205709036)--
(axis cs:26,102750.69253098685)--
(axis cs:25,102738.05269523495)--
(axis cs:24,102748.45996276451)--
(axis cs:23,102752.80421612463)--
(axis cs:22,102746.02621618136)--
(axis cs:21,102744.64805199881)--
(axis cs:20,102745.90626256973)--
(axis cs:19,102718.80602390225)--
(axis cs:18,102733.7011102255)--
(axis cs:17,102731.79696011802)--
(axis cs:16,102733.2828654746)--
(axis cs:15,102718.5203286037)--
(axis cs:14,102720.33158837771)--
(axis cs:13,102712.55932653781)--
(axis cs:12,102711.7936864744)--
(axis cs:11,102694.09869724048)--
(axis cs:10,102681.44403613744)--
(axis cs:9,102676.9447673528)--
(axis cs:8,102668.99162814202)--
(axis cs:7,102647.1845537377)--
(axis cs:6,102648.6957005259)--
(axis cs:5,102619.77979115391)--
(axis cs:4,102584.80460074235)--
(axis cs:3,102556.11718164447)--
(axis cs:2,102446.17053068042)--
(axis cs:1,102263.46617295791)--
cycle;
\addplot [densely dotted, thick, darkorange25512714]
table {%
1 102468.61214634334
2 102593.43129199618
3 102644.87557074614
4 102676.27833225304
5 102700.52204195925
6 102707.77185002175
7 102731.50819471136
8 102746.52500558319
9 102748.67231885079
10 102748.7839811779
11 102755.62415392535
12 102755.04100696015
13 102762.60322113795
14 102769.43006969712
15 102769.27222785201
16 102769.67680724068
17 102772.57417660202
18 102773.18913861841
19 102777.51700231658
20 102774.34864075866
21 102783.16167547973
22 102785.7440072914
23 102780.50624587893
24 102782.15220484074
25 102780.9030411703
26 102784.67668123747
27 102786.69422245209
28 102787.00059924411
29 102788.46642824865
};
% \path [fill=crimson2143940, fill opacity=0.2]
% (axis cs:1,93145.33919676808)--
% (axis cs:1,95461.81870445715)--
% (axis cs:2,95623.87576555365)--
% (axis cs:3,95691.65727427432)--
% (axis cs:4,95671.00918575373)--
% (axis cs:5,95716.0561112232)--
% (axis cs:6,95689.28982318223)--
% (axis cs:7,95723.76175597297)--
% (axis cs:8,95720.64964306998)--
% (axis cs:9,95710.5889107573)--
% (axis cs:10,95708.81397160006)--
% (axis cs:11,95717.39926268478)--
% (axis cs:12,95722.01440655776)--
% (axis cs:13,95717.29199483269)--
% (axis cs:14,95728.6378805985)--
% (axis cs:15,95716.91903288019)--
% (axis cs:16,95724.9154557398)--
% (axis cs:17,95726.80732238619)--
% (axis cs:18,95737.90478258458)--
% (axis cs:19,95732.0247696986)--
% (axis cs:20,95723.96060856615)--
% (axis cs:21,95724.69678859356)--
% (axis cs:22,95725.49996645357)--
% (axis cs:23,95720.77481281798)--
% (axis cs:24,95728.63289767317)--
% (axis cs:25,95725.72593555754)--
% (axis cs:26,95723.28256383061)--
% (axis cs:27,95738.61271909712)--
% (axis cs:28,95734.54436382116)--
% (axis cs:29,95733.83865225822)--
% (axis cs:29,95571.10963120966)--
% (axis cs:28,95581.00404884317)--
% (axis cs:27,95581.36701511135)--
% (axis cs:26,95572.39177646319)--
% (axis cs:25,95542.41734087905)--
% (axis cs:24,95575.24111935052)--
% (axis cs:23,95566.38270843169)--
% (axis cs:22,95540.90595039488)--
% (axis cs:21,95566.81125272623)--
% (axis cs:20,95558.70293612256)--
% (axis cs:19,95551.88176220944)--
% (axis cs:18,95567.74132883504)--
% (axis cs:17,95545.63419801455)--
% (axis cs:16,95533.55523492047)--
% (axis cs:15,95530.91844619214)--
% (axis cs:14,95495.5147147178)--
% (axis cs:13,95502.95977068327)--
% (axis cs:12,95510.24555889372)--
% (axis cs:11,95498.88533922572)--
% (axis cs:10,95515.02949312155)--
% (axis cs:9,95438.00437173009)--
% (axis cs:8,95419.38459129317)--
% (axis cs:7,95475.44900308162)--
% (axis cs:6,95356.88353994612)--
% (axis cs:5,95249.0336475941)--
% (axis cs:4,95161.0495058748)--
% (axis cs:3,95126.75511585517)--
% (axis cs:2,94694.81404531258)--
% (axis cs:1,93145.33919676808)--
% cycle;
% \addplot [dashdotted, thick, crimson2143940]
% table {%
% 1 94821.24646573886
% 2 95339.60663555472
% 3 95510.74816187829
% 4 95521.34327092726
% 5 95570.37625902564
% 6 95562.47973593615
% 7 95604.13199800893
% 8 95595.00657532697
% 9 95618.83067045137
% 10 95634.71225246688
% 11 95622.22130020292
% 12 95636.41176499418
% 13 95626.01087738738
% 14 95639.19021032538
% 15 95635.60583556304
% 16 95646.85025439283
% 17 95650.40959970868
% 18 95669.00836919862
% 19 95651.94325177238
% 20 95654.9884773719
% 21 95653.25423192754
% 22 95645.63844044041
% 23 95654.65307678447
% 24 95669.77773127178
% 25 95643.68427328722
% 26 95654.4608625493
% 27 95657.74753920098
% 28 95659.38053887959
% 29 95660.4122872157
% };
% \path [fill=darkgray176, fill opacity=0.2]
% (axis cs:1,102226.37311332164)--
% (axis cs:1,102647.34019912104)--
% (axis cs:2,102714.56910079812)--
% (axis cs:3,102738.51555060185)--
% (axis cs:4,102748.2455908509)--
% (axis cs:5,102779.45727519973)--
% (axis cs:6,102771.62869115689)--
% (axis cs:7,102783.09457855081)--
% (axis cs:8,102779.74300021688)--
% (axis cs:9,102786.64338314555)--
% (axis cs:10,102792.33674619415)--
% (axis cs:11,102789.54303743184)--
% (axis cs:12,102785.92592068634)--
% (axis cs:13,102791.10179352087)--
% (axis cs:14,102798.35175392526)--
% (axis cs:15,102797.85046163053)--
% (axis cs:16,102806.17182787428)--
% (axis cs:17,102793.10273964361)--
% (axis cs:18,102801.64453717634)--
% (axis cs:19,102805.13418178864)--
% (axis cs:20,102804.05336200935)--
% (axis cs:21,102805.6224592951)--
% (axis cs:22,102802.20136291503)--
% (axis cs:23,102803.78502033837)--
% (axis cs:24,102808.72721503815)--
% (axis cs:25,102808.2038516894)--
% (axis cs:26,102806.28657156961)--
% (axis cs:27,102807.32843134775)--
% (axis cs:28,102805.81079667545)--
% (axis cs:29,102811.25779001026)--
% (axis cs:29,102764.43538540736)--
% (axis cs:28,102757.11285520945)--
% (axis cs:27,102764.04241723898)--
% (axis cs:26,102761.64521505627)--
% (axis cs:25,102749.56305794466)--
% (axis cs:24,102747.2520773782)--
% (axis cs:23,102749.4502493549)--
% (axis cs:22,102742.16484966433)--
% (axis cs:21,102739.78816140689)--
% (axis cs:20,102748.08139206922)--
% (axis cs:19,102741.79420845964)--
% (axis cs:18,102742.24083371574)--
% (axis cs:17,102734.24849826194)--
% (axis cs:16,102735.05310332874)--
% (axis cs:15,102734.30004838147)--
% (axis cs:14,102712.37442978604)--
% (axis cs:13,102713.1043279126)--
% (axis cs:12,102701.16809976212)--
% (axis cs:11,102696.93713920708)--
% (axis cs:10,102693.7391117951)--
% (axis cs:9,102673.56283619025)--
% (axis cs:8,102690.14500288288)--
% (axis cs:7,102658.83755729267)--
% (axis cs:6,102643.71420968593)--
% (axis cs:5,102630.03509497402)--
% (axis cs:4,102591.2422001697)--
% (axis cs:3,102524.31907748622)--
% (axis cs:2,102425.2591390259)--
% (axis cs:1,102226.37311332164)--
% cycle;
% \addplot [thick, darkgray176]
% table {%
% 1 102445.99302529541
% 2 102602.77661225577
% 3 102653.05216480285
% 4 102680.32689815233
% 5 102715.49643394694
% 6 102724.20947818496
% 7 102727.5302864869
% 8 102741.00484090214
% 9 102735.44474222932
% 10 102743.7519176704
% 11 102749.00103554067
% 12 102756.16179785457
% 13 102762.4590889134
% 14 102767.23531733546
% 15 102765.97312100916
% 16 102774.60793847311
% 17 102767.95220411514
% 18 102775.61881292742
% 19 102779.51374086623
% 20 102782.37927651944
% 21 102781.82426749985
% 22 102776.58472070453
% 23 102778.75559285589
% 24 102785.71180617233
% 25 102783.0798137395
% 26 102785.4974399328
% 27 102789.24997153536
% 28 102788.75561838417
% 29 102790.25089236394
% };




==> figures/epsilon/imdb.tex <==
\nextgroupplot [
    title=IMDB,
    xmin=1, xmax=30,
    ymin=98562, ymax=98808,
]

\addplot [dashed, steelblue31119180]
table {%
1 98726
2 98726
3 98726
4 98726
5 98726
6 98726
7 98726
8 98726
9 98726
10 98726
11 98726
12 98726
13 98726
14 98726
15 98726
16 98726
17 98726
18 98726
19 98726
20 98726
21 98726
22 98726
23 98726
24 98726
25 98726
26 98726
27 98726
28 98726
29 98726
};
\path [fill=forestgreen4416044, fill opacity=0.2]
(axis cs:1,98502.21467866922)--
(axis cs:1,98694.50053100802)--
(axis cs:2,98707.22935268877)--
(axis cs:3,98725.17558761415)--
(axis cs:4,98723.49835593153)--
(axis cs:5,98723.79180480713)--
(axis cs:6,98725.36551091739)--
(axis cs:7,98726.8553434981)--
(axis cs:8,98725.86744209583)--
(axis cs:9,98723.82629390858)--
(axis cs:10,98724.97811766232)--
(axis cs:11,98722.44120228948)--
(axis cs:12,98727.20795936539)--
(axis cs:13,98725.62036140868)--
(axis cs:14,98726.90065760924)--
(axis cs:15,98727.81559212154)--
(axis cs:16,98726.12218785126)--
(axis cs:17,98726.12565521365)--
(axis cs:18,98726.8034924029)--
(axis cs:19,98726.95646020856)--
(axis cs:20,98726.28932629185)--
(axis cs:21,98726.01269685556)--
(axis cs:22,98727.05634480318)--
(axis cs:23,98726.38328055275)--
(axis cs:24,98726.83491823863)--
(axis cs:25,98726.58334357924)--
(axis cs:26,98726.92208416267)--
(axis cs:27,98725.67596336371)--
(axis cs:28,98725.88110054182)--
(axis cs:29,98726.2012542949)--
(axis cs:29,98718.28257133042)--
(axis cs:28,98717.55563777719)--
(axis cs:27,98716.64801313328)--
(axis cs:26,98713.93415610185)--
(axis cs:25,98717.16520726)--
(axis cs:24,98717.46510040628)--
(axis cs:23,98714.85485967057)--
(axis cs:22,98710.754705055)--
(axis cs:21,98716.69707968207)--
(axis cs:20,98715.26012799457)--
(axis cs:19,98710.05666948529)--
(axis cs:18,98709.85577803844)--
(axis cs:17,98706.32424450095)--
(axis cs:16,98710.21841864202)--
(axis cs:15,98708.52426954421)--
(axis cs:14,98708.56139188314)--
(axis cs:13,98704.50685797937)--
(axis cs:12,98700.83648650693)--
(axis cs:11,98698.442337955)--
(axis cs:10,98701.64134178364)--
(axis cs:9,98699.3964555292)--
(axis cs:8,98701.37049094359)--
(axis cs:7,98688.85488082872)--
(axis cs:6,98682.25107216595)--
(axis cs:5,98676.45864160285)--
(axis cs:4,98652.84231626216)--
(axis cs:3,98628.13499458517)--
(axis cs:2,98590.47450839348)--
(axis cs:1,98502.21467866922)--
cycle;
\addplot [densely dotted, thick, forestgreen4416044]
table {%
1 98624.75992511184
2 98659.3533337554
3 98686.77805187504
4 98697.02390247132
5 98704.35770642327
6 98710.89525414669
7 98711.68614380024
8 98715.08804410299
9 98716.77950780754
10 98717.36835842094
11 98715.13527638392
12 98717.97044351185
13 98717.46171840877
14 98719.1909899259
15 98719.91129239321
16 98720.59681014666
17 98719.86567567269
18 98720.878568013
19 98721.63962482577
20 98721.38806705986
21 98721.8052369938
22 98721.53654570034
23 98722.09757031119
24 98723.24002648237
25 98722.36712302294
26 98722.58694184638
27 98723.11946691187
28 98723.38462294888
29 98723.51426389045
};
\path [fill=darkorange25512714, fill opacity=0.2]
(axis cs:1,98505.67637468634)--
(axis cs:1,98705.05457934595)--
(axis cs:2,98730.34014654763)--
(axis cs:3,98726.08102052263)--
(axis cs:4,98724.40549991307)--
(axis cs:5,98719.49124760118)--
(axis cs:6,98722.76189295347)--
(axis cs:7,98727.01863405439)--
(axis cs:8,98725.09306286076)--
(axis cs:9,98724.03637904025)--
(axis cs:10,98725.53769523882)--
(axis cs:11,98727.2304059918)--
(axis cs:12,98724.76542948125)--
(axis cs:13,98725.21828407959)--
(axis cs:14,98725.32846317261)--
(axis cs:15,98726.86137341587)--
(axis cs:16,98729.8755258522)--
(axis cs:17,98725.35268452518)--
(axis cs:18,98726.52827257612)--
(axis cs:19,98726.26548289252)--
(axis cs:20,98727.21575606446)--
(axis cs:21,98728.36936468215)--
(axis cs:22,98726.39119377478)--
(axis cs:23,98726.67879695602)--
(axis cs:24,98726.81605098284)--
(axis cs:25,98727.87445710486)--
(axis cs:26,98725.9807078872)--
(axis cs:27,98726.256960183)--
(axis cs:28,98726.82218833499)--
(axis cs:29,98726.03037614276)--
(axis cs:29,98716.51749224792)--
(axis cs:28,98716.98809784684)--
(axis cs:27,98713.22549183707)--
(axis cs:26,98712.35535890129)--
(axis cs:25,98714.11059256356)--
(axis cs:24,98715.1193093968)--
(axis cs:23,98712.2355999502)--
(axis cs:22,98712.70503171092)--
(axis cs:21,98711.70359655586)--
(axis cs:20,98714.4474839096)--
(axis cs:19,98710.76031628254)--
(axis cs:18,98712.1645712603)--
(axis cs:17,98708.66565694768)--
(axis cs:16,98709.27439324286)--
(axis cs:15,98706.80707274412)--
(axis cs:14,98703.00674412932)--
(axis cs:13,98705.46063949591)--
(axis cs:12,98703.08579856192)--
(axis cs:11,98695.86972608705)--
(axis cs:10,98698.15638863955)--
(axis cs:9,98691.75503108054)--
(axis cs:8,98686.09427648966)--
(axis cs:7,98688.12905815471)--
(axis cs:6,98668.35779600932)--
(axis cs:5,98665.3938181446)--
(axis cs:4,98648.20865436352)--
(axis cs:3,98635.67154794792)--
(axis cs:2,98588.43743006107)--
(axis cs:1,98505.67637468634)--
cycle;
\addplot [densely dotted, thick, darkorange25512714]
table {%
1 98610.12874900417
2 98673.18044521978
3 98693.7662712342
4 98694.20674607529
5 98699.2045658798
6 98707.17488707155
7 98709.211946498
8 98714.97702982137
9 98713.64773673133
10 98715.40016631596
11 98716.76447376737
12 98717.38220810125
13 98718.77711861569
14 98718.96042628639
15 98719.38579496363
16 98721.58401327473
17 98719.72184475715
18 98720.79249168535
19 98720.06822311587
20 98722.03388942113
21 98722.01683505594
22 98721.80650506439
23 98721.49393201471
24 98722.33632622077
25 98722.83180647204
26 98721.9633209988
27 98722.58496479012
28 98721.81642411236
29 98722.43191772007
};
% \path [fill=crimson2143940, fill opacity=0.2]
% (axis cs:1,79088.09583401842)--
% (axis cs:1,81001.54822356859)--
% (axis cs:2,81057.28856512335)--
% (axis cs:3,81114.7126966959)--
% (axis cs:4,81146.84463169452)--
% (axis cs:5,81118.35574886118)--
% (axis cs:6,81127.07996902068)--
% (axis cs:7,81081.72477837715)--
% (axis cs:8,81143.3934030974)--
% (axis cs:9,81181.04440300865)--
% (axis cs:10,81134.95139124649)--
% (axis cs:11,81169.93694047017)--
% (axis cs:12,81132.17854350012)--
% (axis cs:13,81124.7095572727)--
% (axis cs:14,81183.60348923414)--
% (axis cs:15,81175.53368782288)--
% (axis cs:16,81150.60640023556)--
% (axis cs:17,81125.66816050929)--
% (axis cs:18,81150.21648986232)--
% (axis cs:19,81134.94614085811)--
% (axis cs:20,81150.21423486203)--
% (axis cs:21,81169.53708700284)--
% (axis cs:22,81163.12876535967)--
% (axis cs:23,81123.03590550616)--
% (axis cs:24,81148.4017379182)--
% (axis cs:25,81145.40490127692)--
% (axis cs:26,81163.1804675035)--
% (axis cs:27,81196.07955949282)--
% (axis cs:28,81157.32742402589)--
% (axis cs:29,81170.62252448993)--
% (axis cs:29,80941.96089901232)--
% (axis cs:28,80929.29240863804)--
% (axis cs:27,80930.7880826013)--
% (axis cs:26,80933.52873934829)--
% (axis cs:25,80957.75584357134)--
% (axis cs:24,80936.82431216248)--
% (axis cs:23,80914.5541518496)--
% (axis cs:22,80944.21375343602)--
% (axis cs:21,80928.16083199647)--
% (axis cs:20,80913.66683840586)--
% (axis cs:19,80890.4260064007)--
% (axis cs:18,80906.04100234709)--
% (axis cs:17,80907.96809647321)--
% (axis cs:16,80896.71748907755)--
% (axis cs:15,80911.82247232209)--
% (axis cs:14,80893.72216044506)--
% (axis cs:13,80903.402243641)--
% (axis cs:12,80915.25235199477)--
% (axis cs:11,80750.31335810633)--
% (axis cs:10,80835.791509776)--
% (axis cs:9,80858.34573129524)--
% (axis cs:8,80803.77820533117)--
% (axis cs:7,80765.71307088684)--
% (axis cs:6,80779.30741503858)--
% (axis cs:5,80704.62758717738)--
% (axis cs:4,80600.91111223707)--
% (axis cs:3,80518.9703039717)--
% (axis cs:2,79978.65992726227)--
% (axis cs:1,79088.09583401842)--
% cycle;
% \addplot [dashdotted, thick, crimson2143940]
% table {%
% 1 80236.42813974629
% 2 80688.24290846699
% 3 80908.91974346444
% 4 80968.51570516237
% 5 80946.8933996283
% 6 80991.40216445502
% 7 80964.2039986759
% 8 81012.1619585482
% 9 81009.36015591791
% 10 81012.86457332221
% 11 81013.09366196775
% 12 81017.92690852522
% 13 81020.97915031872
% 14 81028.25450260614
% 15 81038.62037105905
% 16 81029.71372322013
% 17 81025.44715811926
% 18 81032.13544855022
% 19 81022.17765012084
% 20 81026.29220062312
% 21 81020.67830739928
% 22 81024.09400021998
% 23 81013.06904629893
% 24 81038.1560343756
% 25 81031.24746818568
% 26 81027.41309535864
% 27 81026.45884038831
% 28 81024.06965451688
% 29 81037.05429870672
% };
% \path [fill=darkgray176, fill opacity=0.2]
% (axis cs:1,98431.53215570883)--
% (axis cs:1,98764.30557676281)--
% (axis cs:2,98717.64206424911)--
% (axis cs:3,98736.91575718933)--
% (axis cs:4,98724.25399607488)--
% (axis cs:5,98725.63765531576)--
% (axis cs:6,98724.00953530392)--
% (axis cs:7,98725.91419427551)--
% (axis cs:8,98725.28400075535)--
% (axis cs:9,98728.12186861246)--
% (axis cs:10,98732.03759017738)--
% (axis cs:11,98729.96027617874)--
% (axis cs:12,98723.42624562478)--
% (axis cs:13,98726.58818391811)--
% (axis cs:14,98724.7464159837)--
% (axis cs:15,98725.91495157205)--
% (axis cs:16,98725.99452046929)--
% (axis cs:17,98724.29506225046)--
% (axis cs:18,98726.83595997785)--
% (axis cs:19,98727.96954916563)--
% (axis cs:20,98727.09471971139)--
% (axis cs:21,98726.49297921911)--
% (axis cs:22,98724.97924060753)--
% (axis cs:23,98727.19498246138)--
% (axis cs:24,98727.84517206944)--
% (axis cs:25,98725.85529059163)--
% (axis cs:26,98726.44092930082)--
% (axis cs:27,98728.10756062788)--
% (axis cs:28,98725.85103453157)--
% (axis cs:29,98726.07264483171)--
% (axis cs:29,98711.47938576926)--
% (axis cs:28,98716.22597104155)--
% (axis cs:27,98716.97725254844)--
% (axis cs:26,98714.62793812953)--
% (axis cs:25,98716.67821142072)--
% (axis cs:24,98714.56824056449)--
% (axis cs:23,98715.94299463328)--
% (axis cs:22,98714.53613025742)--
% (axis cs:21,98712.49414391213)--
% (axis cs:20,98709.6653181348)--
% (axis cs:19,98712.81048493189)--
% (axis cs:18,98710.97810284841)--
% (axis cs:17,98709.19114959861)--
% (axis cs:16,98707.27520661782)--
% (axis cs:15,98705.0421037197)--
% (axis cs:14,98704.65211736159)--
% (axis cs:13,98705.11292827701)--
% (axis cs:12,98697.54819889778)--
% (axis cs:11,98702.42383884452)--
% (axis cs:10,98693.65964445123)--
% (axis cs:9,98693.11641724738)--
% (axis cs:8,98686.16085319918)--
% (axis cs:7,98690.44702012466)--
% (axis cs:6,98661.72134125743)--
% (axis cs:5,98663.29135615)--
% (axis cs:4,98652.76123031812)--
% (axis cs:3,98611.38448401725)--
% (axis cs:2,98566.1917370303)--
% (axis cs:1,98431.53215570883)--
% cycle;
% \addplot [thick, darkgray176]
% table {%
% 1 98624.5994904149
% 2 98667.40945751179
% 3 98692.08053476244
% 4 98694.46767312312
% 5 98703.92010403943
% 6 98709.07703345637
% 7 98711.66260923272
% 8 98712.51105600156
% 9 98715.1850525497
% 10 98716.48034726636
% 11 98716.17890619753
% 12 98715.5188419811
% 13 98718.14940482759
% 14 98719.0887632946
% 15 98718.68357305744
% 16 98719.90661778081
% 17 98718.95977505528
% 18 98721.0578984067
% 19 98721.40302161666
% 20 98720.9780766591
% 21 98720.6378896379
% 22 98721.06569896116
% 23 98722.40108637628
% 24 98721.17764856943
% 25 98721.84412228907
% 26 98721.87012541937
% 27 98722.97309931445
% 28 98722.85662796911
% 29 98722.49216190695
% };



